Explainable Benchmarking for Iterative Optimization Heuristics

Benchmarking heuristic algorithms is vital to understand under which conditions and on what kind of problems certain algorithms perform well. In most current research into heuristic optimization algorithms, only a very limited number of scenarios, algorithm configurations and hyper-parameter settings are explored, leading to incomplete and often biased insights and results. This paper presents a novel approach we call explainable benchmarking. Introducing the IOH-Xplainer software framework, for analyzing and understanding the performance of various optimization algorithms and the impact of their different components and hyper-parameters. We showcase the framework in the context of two modular optimization frameworks. Through this framework, we examine the impact of different algorithmic components and configurations, offering insights into their performance across diverse scenarios. We provide a systematic method for evaluating and interpreting the behaviour and efficiency of iterative optimization heuristics in a more transparent and comprehensible manner, allowing for better benchmarking and algorithm design.

==> Biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{diederick.jpg}}]{Diederick Vermetten} is a Phd Candidate at Leiden University (NL), where he is part of the NaCo group.
% He is supervised by Hao Wang and Thomas B\"ack from Leiden University and Carola Doerr from Sorbonne University, CNRS. 
His research interests include benchmarking of optimisation heuristics, dynamic algorithm selection and configuration as well as hyperparameter optimisation. He is a part of the core development team of the IOHprofiler project for benchmarking iterative optimisation heuristics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bas.jpeg}}]{Bas van Stein} (M'22) received his Ph.D. degree in Computer Science in 2018, from the Leiden Institute of Advanced Computer Science (LIACS), Leiden University, The Netherlands.

From 2018 until 2021 he was a Postdoctoral Researcher at LIACS, Leiden University and he is currently an Assistant Professor at LIACS. His research interests lie in surrogate assisted optimisation, surrogate assisted neural architecture search and explainable AI techniques for industrial applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author_Photos/fabio.jpg}}]{Fabio Caraffini} is currently an Associate Professor in Computer Science at De Montfort University (UK), where he is a member of the Institute of Artificial Intelligence. He received the BSc in ``Electronics Engineering'' and the MSc in ``Telecommunications Engineering'' degrees from the University of Perugia (Italy) in 2008 and 2011 respectively, and holds a PhD in Computer Science (De Montfort University, UK, 2014) and a PhD in Mathematical Information Technology (University of Jyv\"askyl\"a, Finland, 2016). His research interests include theoretical and applied computational intelligence with a strong emphasis on metaheuristics for optimisation. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Minku.jpg}}]{Leandro L. Minku} is an Associate Professor at the University of Birmingham (UK). Prior to that, he was a Lecturer (Assistant Professor) at the University of Leicester (UK). He received the PhD degree in Computer Science from the University of Birmingham (UK) in 2010. Among other roles, Dr. Minku is Associate Editor-in-Chief for Neurocomputing, Senior Editor for IEEE Transactions on Neural Networks and Learning Systems, Associate Editor for Empirical Software Engineering Journal, and Associate Editor for Journal of Systems and Software. Dr. Minku's main research interests are machine learning for non-stationary environments / data stream learning, class imbalance learning, ensembles of learning machines, dynamic optimisation and computational intelligence for software engineering. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Anna.png}}]{Anna V. Kononova} (M'04) is currently an Assistant Professor at the Leiden Institute of Advanced Computer Science (The Netherlands). She received her MSc degree in Applied Mathematics from Yaroslavl State University (Russia) in 2004 and her PhD degree in Computer Science from University of Leeds (UK) in 2010. After 5 years of postdoctoral experience at Technical University Eindhoven (Netherlands) and Heriot-Watt University (Edinburgh, UK), Anna spent 5 years working as an engineer and a mathematician in industry. Her current research interests include analysis of behaviour of optimisation algorithms and machine learning.
\end{IEEEbiography}

==> hallOfFame/cma.tex <==
\begin{tabular}{rrrrlllllrrr}
\toprule
dim & fid & covariance & elitist & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & lambda_ & mu & auc \\
\midrule
5 & 1 & True & True & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.985746 \\
5 & 1 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.983376 \\
5 & 1 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.984011 \\
5 & 1 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.984186 \\
5 & 1 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.985330 \\
5 & 2 & False & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.908018 \\
5 & 2 & False & True & mirrored & sobol & equal & IPOP & psr & 5.000000 & 5.000000 & 0.916046 \\
5 & 2 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 10.000000 & 5.000000 & 0.907917 \\
5 & 2 & False & False & mirrored & sobol & 1/2^lambda & IPOP & csa & 8.000000 & 5.000000 & 0.905143 \\
5 & 2 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.926029 \\
5 & 3 & False & False & mirrored & halton & default & BIPOP & csa & 8.000000 & 3.000000 & 0.955587 \\
5 & 3 & False & False & mirrored & halton & default & BIPOP & csa & 20.000000 & 5.000000 & 0.924649 \\
5 & 3 & True & False & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 10.000000 & 10.000000 & 0.914860 \\
5 & 3 & False & False & mirrored & halton & default & BIPOP & csa & 8.000000 & 3.000000 & 0.953675 \\
5 & 3 & True & False & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 5.000000 & 0.940028 \\
5 & 4 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.951676 \\
5 & 4 & False & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 10.000000 & 5.000000 & 0.195147 \\
5 & 4 & True & True & mirrored pairwise & gaussian & default & BIPOP & psr & 8.000000 & 3.000000 & 0.370171 \\
5 & 4 & True & True & mirrored & gaussian & default & IPOP & psr & 10.000000 & 5.000000 & 0.344063 \\
5 & 4 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & psr & 10.000000 & 5.000000 & 0.192925 \\
5 & 5 & True & True & mirrored & halton & default & BIPOP & psr & 5.000000 & 5.000000 & 0.998441 \\
5 & 5 & True & False & mirrored & gaussian & default & IPOP & csa & 5.000000 & 5.000000 & 0.998863 \\
5 & 5 & True & True & mirrored & gaussian & default & IPOP & csa & 5.000000 & 5.000000 & 0.998398 \\
5 & 5 & False & False & mirrored & halton & default & BIPOP & psr & 5.000000 & 5.000000 & 0.998448 \\
5 & 5 & True & False & mirrored pairwise & halton & default & BIPOP & psr & 5.000000 & 2.000000 & 0.998248 \\
5 & 6 & True & True & mirrored pairwise & sobol & equal & IPOP & csa & 5.000000 & 2.000000 & 0.962468 \\
5 & 6 & True & True & mirrored & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.964399 \\
5 & 6 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.964264 \\
5 & 6 & True & True & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.962085 \\
5 & 6 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.957602 \\
5 & 7 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 10.000000 & 5.000000 & 0.975450 \\
5 & 7 & False & False & mirrored & halton & default & BIPOP & csa & 8.000000 & 3.000000 & 0.984475 \\
5 & 7 & False & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 5.000000 & 2.000000 & 0.983970 \\
5 & 7 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 8.000000 & 5.000000 & 0.983863 \\
5 & 7 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.982403 \\
5 & 8 & True & True & mirrored & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.933890 \\
5 & 8 & True & True & mirrored pairwise & halton & default & BIPOP & csa & 8.000000 & 5.000000 & 0.941061 \\
5 & 8 & True & True & mirrored pairwise & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.943660 \\
5 & 8 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.956613 \\
5 & 8 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.934046 \\
5 & 9 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.953205 \\
5 & 9 & True & True & mirrored & halton & default & BIPOP & csa & 8.000000 & 5.000000 & 0.941204 \\
5 & 9 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 2.000000 & 0.938959 \\
5 & 9 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 5.000000 & 0.950800 \\
5 & 9 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 2.000000 & 0.946881 \\
5 & 10 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 5.000000 & 0.915513 \\
5 & 10 & True & True & mirrored & sobol & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.912127 \\
5 & 10 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 5.000000 & 5.000000 & 0.924213 \\
5 & 10 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.922890 \\
5 & 10 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.910334 \\
5 & 11 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.921611 \\
5 & 11 & True & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.918034 \\
5 & 11 & True & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.923247 \\
5 & 11 & True & False & mirrored & halton & default & BIPOP & csa & 20.000000 & 10.000000 & 0.917747 \\
5 & 11 & True & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.926030 \\
5 & 12 & True & True & mirrored pairwise & halton & default & BIPOP & csa & 8.000000 & 5.000000 & 0.890588 \\
5 & 12 & True & True & mirrored & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.912906 \\
5 & 12 & False & False & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.867408 \\
5 & 12 & True & True & mirrored & sobol & default & IPOP & csa & 5.000000 & 2.000000 & 0.912928 \\
5 & 12 & True & True & mirrored & halton & equal & BIPOP & csa & 10.000000 & 5.000000 & 0.919694 \\
5 & 13 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.913151 \\
5 & 13 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 5.000000 & 0.906093 \\
5 & 13 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.912642 \\
5 & 13 & False & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.917558 \\
5 & 13 & True & True & mirrored & halton & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.907090 \\
5 & 14 & True & False & mirrored & halton & default & BIPOP & csa & 20.000000 & 10.000000 & 0.960950 \\
5 & 14 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 8.000000 & 5.000000 & 0.957796 \\
5 & 14 & True & True & mirrored pairwise & sobol & equal & IPOP & csa & 5.000000 & 5.000000 & 0.960511 \\
5 & 14 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 8.000000 & 3.000000 & 0.953990 \\
5 & 14 & True & True & mirrored pairwise & sobol & equal & IPOP & csa & 5.000000 & 5.000000 & 0.955484 \\
5 & 15 & False & False & mirrored pairwise & halton & equal & BIPOP & psr & 5.000000 & 2.000000 & 0.919109 \\
5 & 15 & False & False & mirrored & halton & equal & BIPOP & csa & 8.000000 & 3.000000 & 0.932574 \\
5 & 15 & False & False & mirrored & halton & equal & BIPOP & csa & 20.000000 & 5.000000 & 0.914281 \\
5 & 15 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.962968 \\
5 & 15 & False & False & mirrored & halton & default & BIPOP & psr & 8.000000 & 3.000000 & 0.950178 \\
5 & 16 & False & False & mirrored & halton & default & BIPOP & psr & 8.000000 & 5.000000 & 0.958264 \\
5 & 16 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 8.000000 & 3.000000 & 0.961799 \\
5 & 16 & True & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.958347 \\
5 & 16 & True & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 10.000000 & 5.000000 & 0.947457 \\
5 & 16 & True & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 8.000000 & 5.000000 & 0.962415 \\
5 & 17 & False & False & mirrored & halton & default & BIPOP & csa & 8.000000 & 3.000000 & 0.940554 \\
5 & 17 & False & False & mirrored & halton & default & BIPOP & csa & 10.000000 & 5.000000 & 0.946945 \\
5 & 17 & False & False & mirrored & halton & default & BIPOP & csa & 10.000000 & 5.000000 & 0.940975 \\
5 & 17 & True & False & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.936331 \\
5 & 17 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.943350 \\
5 & 18 & True & False & mirrored & halton & default & BIPOP & csa & 20.000000 & 10.000000 & 0.912651 \\
5 & 18 & True & True & mirrored & halton & equal & BIPOP & csa & 10.000000 & 10.000000 & 0.936322 \\
5 & 18 & False & False & mirrored & halton & default & BIPOP & psr & 20.000000 & 10.000000 & 0.897103 \\
5 & 18 & False & False & mirrored & halton & default & BIPOP & csa & 10.000000 & 5.000000 & 0.931898 \\
5 & 18 & True & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 10.000000 & 5.000000 & 0.917064 \\
5 & 19 & False & False & mirrored pairwise & halton & equal & BIPOP & csa & 20.000000 & 5.000000 & 0.866734 \\
5 & 19 & True & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 5.000000 & 0.925071 \\
5 & 19 & False & False & mirrored & halton & default & BIPOP & csa & 8.000000 & 5.000000 & 0.847109 \\
5 & 19 & True & False & mirrored & halton & equal & BIPOP & csa & 8.000000 & 5.000000 & 0.821826 \\
5 & 19 & True & False & mirrored & sobol & 1/2^lambda & BIPOP & psr & 20.000000 & 5.000000 & 0.670749 \\
5 & 20 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.866103 \\
5 & 20 & True & True & mirrored pairwise & halton & default & BIPOP & csa & 20.000000 & 5.000000 & 0.918321 \\
5 & 20 & True & True & mirrored & halton & default & BIPOP & csa & 20.000000 & 5.000000 & 0.705118 \\
5 & 20 & True & False & mirrored pairwise & sobol & 1/2^lambda & IPOP & csa & 20.000000 & 20.000000 & 0.557196 \\
5 & 20 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.860639 \\
5 & 21 & True & True & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.987790 \\
5 & 21 & True & True & mirrored pairwise & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.986815 \\
5 & 21 & False & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 5.000000 & 5.000000 & 0.988300 \\
5 & 21 & True & True & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.986687 \\
5 & 21 & True & True & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 2.000000 & 0.987595 \\
5 & 22 & True & False & mirrored & halton & equal & BIPOP & psr & 8.000000 & 3.000000 & 0.982900 \\
5 & 22 & False & True & mirrored pairwise & halton & equal & BIPOP & psr & 8.000000 & 3.000000 & 0.969315 \\
5 & 22 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 2.000000 & 0.971066 \\
5 & 22 & True & True & mirrored & sobol & default & IPOP & csa & 8.000000 & 3.000000 & 0.966728 \\
5 & 22 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.977229 \\
5 & 23 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.913901 \\
5 & 23 & True & False & mirrored & halton & default & IPOP & csa & 10.000000 & 5.000000 & 0.891482 \\
5 & 23 & True & False & mirrored & halton & default & BIPOP & psr & 8.000000 & 5.000000 & 0.896681 \\
5 & 23 & False & False & mirrored & halton & default & BIPOP & csa & 5.000000 & 2.000000 & 0.902645 \\
5 & 23 & False & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 20.000000 & 10.000000 & 0.809445 \\
5 & 24 & True & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 8.000000 & 3.000000 & 0.205588 \\
5 & 24 & False & False & mirrored pairwise & halton & default & BIPOP & csa & 10.000000 & 5.000000 & 0.238669 \\
5 & 24 & True & False & mirrored pairwise & halton & 1/2^lambda & BIPOP & psr & 5.000000 & 5.000000 & 0.213210 \\
5 & 24 & True & False & mirrored & sobol & equal & BIPOP & psr & 20.000000 & 5.000000 & 0.214223 \\
5 & 24 & True & True & mirrored pairwise & halton & default & IPOP & csa & 5.000000 & 5.000000 & 0.177961 \\
30 & 1 & False & False & mirrored & sobol & 1/2^lambda & BIPOP & psr & 5.000000 & 5.000000 & 0.913110 \\
30 & 1 & False & False & mirrored & sobol & 1/2^lambda & BIPOP & psr & 5.000000 & 5.000000 & 0.912908 \\
30 & 1 & False & False & mirrored & sobol & 1/2^lambda & IPOP & psr & 5.000000 & 5.000000 & 0.915686 \\
30 & 1 & False & False & mirrored & sobol & 1/2^lambda & IPOP & psr & 5.000000 & 5.000000 & 0.912426 \\
30 & 1 & False & False & mirrored & sobol & 1/2^lambda & BIPOP & psr & 5.000000 & 5.000000 & 0.912713 \\
30 & 2 & True & True & mirrored & sobol & equal & BIPOP & psr & 10.000000 & 10.000000 & 0.001085 \\
30 & 2 & False & True & mirrored pairwise & gaussian & equal & IPOP & psr & 10.000000 & 10.000000 & 0.004396 \\
30 & 2 & True & True & mirrored & gaussian & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.002436 \\
30 & 2 & True & True & mirrored pairwise & sobol & equal & IPOP & psr & 10.000000 & 10.000000 & 0.002673 \\
30 & 2 & False & True & mirrored pairwise & sobol & equal & IPOP & psr & 10.000000 & 10.000000 & 0.002383 \\
30 & 3 & True & False & mirrored & gaussian & default & IPOP & psr & 20.000000 & 10.000000 & 0.048617 \\
30 & 3 & True & False & mirrored & sobol & equal & IPOP & psr & 20.000000 & 10.000000 & 0.051728 \\
30 & 3 & True & True & mirrored pairwise & gaussian & equal & BIPOP & psr & 20.000000 & 20.000000 & 0.051086 \\
30 & 3 & True & True & mirrored pairwise & sobol & equal & IPOP & psr & 20.000000 & 20.000000 & 0.045651 \\
30 & 3 & False & False & mirrored & sobol & default & BIPOP & psr & 20.000000 & 10.000000 & 0.046023 \\
30 & 4 & False & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.025540 \\
30 & 4 & False & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.031532 \\
30 & 4 & True & False & mirrored pairwise & sobol & default & BIPOP & csa & 20.000000 & 5.000000 & 0.025955 \\
30 & 4 & True & False & mirrored pairwise & sobol & default & IPOP & csa & 20.000000 & 5.000000 & 0.027066 \\
30 & 4 & True & False & mirrored pairwise & sobol & equal & BIPOP & csa & 20.000000 & 5.000000 & 0.024747 \\
30 & 5 & True & True & mirrored & sobol & default & IPOP & psr & 5.000000 & 5.000000 & 0.991667 \\
30 & 5 & True & True & mirrored & halton & default & BIPOP & psr & 5.000000 & 5.000000 & 0.996500 \\
30 & 5 & True & True & mirrored & halton & default & BIPOP & psr & 5.000000 & 5.000000 & 0.996500 \\
30 & 5 & True & True & mirrored & gaussian & default & IPOP & psr & 5.000000 & 5.000000 & 0.990167 \\
30 & 5 & True & True & mirrored & sobol & default & BIPOP & psr & 5.000000 & 5.000000 & 0.988667 \\
30 & 6 & False & False & mirrored pairwise & sobol & 1/2^lambda & IPOP & psr & 14.000000 & 10.000000 & 0.387734 \\
30 & 6 & False & False & mirrored & sobol & default & IPOP & csa & 14.000000 & 4.000000 & 0.364246 \\
30 & 6 & False & False & mirrored & sobol & default & IPOP & csa & 14.000000 & 5.000000 & 0.345843 \\
30 & 6 & True & False & mirrored & gaussian & default & IPOP & csa & 14.000000 & 4.000000 & 0.348098 \\
30 & 6 & False & False & mirrored pairwise & sobol & 1/2^lambda & IPOP & psr & 14.000000 & 5.000000 & 0.356368 \\
30 & 7 & True & False & mirrored & halton & default & BIPOP & csa & 20.000000 & 10.000000 & 0.139411 \\
30 & 7 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.135317 \\
30 & 7 & False & False & mirrored & sobol & 1/2^lambda & BIPOP & csa & 14.000000 & 4.000000 & 0.133556 \\
30 & 7 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.131949 \\
30 & 7 & True & False & mirrored pairwise & sobol & 1/2^lambda & BIPOP & csa & 14.000000 & 5.000000 & 0.124208 \\
30 & 8 & False & False & mirrored & sobol & equal & IPOP & csa & 14.000000 & 4.000000 & 0.093936 \\
30 & 8 & False & False & mirrored & halton & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.097384 \\
30 & 8 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.067791 \\
30 & 8 & True & True & mirrored pairwise & gaussian & equal & BIPOP & csa & 5.000000 & 5.000000 & 0.095442 \\
30 & 8 & True & True & mirrored & gaussian & default & IPOP & csa & 5.000000 & 2.000000 & 0.072582 \\
30 & 9 & True & True & mirrored & gaussian & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.075602 \\
30 & 9 & True & True & mirrored pairwise & gaussian & equal & IPOP & csa & 5.000000 & 2.000000 & 0.070891 \\
30 & 9 & False & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 20.000000 & 10.000000 & 0.078071 \\
30 & 9 & True & False & mirrored & gaussian & 1/2^lambda & IPOP & csa & 5.000000 & 2.000000 & 0.108416 \\
30 & 9 & True & False & mirrored & sobol & default & IPOP & psr & 5.000000 & 2.000000 & 0.088532 \\
30 & 10 & False & True & mirrored & sobol & equal & IPOP & psr & 5.000000 & 5.000000 & 0.000606 \\
30 & 10 & False & True & mirrored pairwise & sobol & equal & IPOP & psr & 10.000000 & 10.000000 & 0.002104 \\
30 & 10 & False & True & mirrored & sobol & equal & BIPOP & psr & 5.000000 & 5.000000 & 0.000945 \\
30 & 10 & False & True & mirrored & gaussian & equal & IPOP & psr & 10.000000 & 10.000000 & 0.003439 \\
30 & 10 & False & True & mirrored pairwise & sobol & equal & IPOP & psr & 10.000000 & 10.000000 & 0.003047 \\
30 & 11 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.079524 \\
30 & 11 & True & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.069794 \\
30 & 11 & True & False & mirrored & sobol & default & IPOP & csa & 14.000000 & 4.000000 & 0.067758 \\
30 & 11 & True & False & mirrored & sobol & default & BIPOP & psr & 10.000000 & 5.000000 & 0.068981 \\
30 & 11 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.067893 \\
30 & 12 & False & False & mirrored & gaussian & equal & IPOP & psr & 5.000000 & 2.000000 & 0.326908 \\
30 & 12 & True & True & mirrored & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.387242 \\
30 & 12 & False & False & mirrored pairwise & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 2.000000 & 0.364180 \\
30 & 12 & False & False & mirrored pairwise & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.359034 \\
30 & 12 & True & True & mirrored & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.446769 \\
30 & 13 & True & True & mirrored pairwise & halton & 1/2^lambda & BIPOP & csa & 10.000000 & 5.000000 & 0.315950 \\
30 & 13 & False & False & mirrored & sobol & equal & IPOP & csa & 20.000000 & 10.000000 & 0.306472 \\
30 & 13 & True & False & mirrored pairwise & sobol & 1/2^lambda & IPOP & csa & 5.000000 & 5.000000 & 0.326420 \\
30 & 13 & True & False & mirrored pairwise & gaussian & 1/2^lambda & IPOP & csa & 10.000000 & 10.000000 & 0.313354 \\
30 & 13 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.305833 \\
30 & 14 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.531639 \\
30 & 14 & True & True & mirrored & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.528920 \\
30 & 14 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.536726 \\
30 & 14 & True & True & mirrored & gaussian & 1/2^lambda & IPOP & csa & 5.000000 & 5.000000 & 0.533419 \\
30 & 14 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.528511 \\
30 & 15 & False & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.055853 \\
30 & 15 & False & False & mirrored & sobol & default & IPOP & psr & 20.000000 & 10.000000 & 0.048947 \\
30 & 15 & True & True & mirrored pairwise & sobol & equal & IPOP & psr & 20.000000 & 20.000000 & 0.052780 \\
30 & 15 & False & False & mirrored & gaussian & default & IPOP & csa & 20.000000 & 10.000000 & 0.052131 \\
30 & 15 & True & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.051273 \\
30 & 16 & True & False & mirrored & sobol & default & IPOP & csa & 14.000000 & 10.000000 & 0.212354 \\
30 & 16 & False & False & mirrored pairwise & sobol & equal & BIPOP & psr & 20.000000 & 5.000000 & 0.211537 \\
30 & 16 & False & False & mirrored pairwise & sobol & default & IPOP & psr & 14.000000 & 4.000000 & 0.211708 \\
30 & 16 & False & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.214507 \\
30 & 16 & False & False & mirrored & sobol & default & IPOP & psr & 20.000000 & 20.000000 & 0.218287 \\
30 & 17 & True & False & mirrored pairwise & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.424696 \\
30 & 17 & False & False & mirrored & sobol & default & BIPOP & psr & 20.000000 & 10.000000 & 0.410282 \\
30 & 17 & False & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.425124 \\
30 & 17 & False & False & mirrored & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.466273 \\
30 & 17 & False & False & mirrored & sobol & default & BIPOP & csa & 14.000000 & 4.000000 & 0.441932 \\
30 & 18 & False & False & mirrored pairwise & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.299606 \\
30 & 18 & False & False & mirrored pairwise & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.300902 \\
30 & 18 & False & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.300664 \\
30 & 18 & True & False & mirrored pairwise & sobol & default & BIPOP & csa & 20.000000 & 10.000000 & 0.303459 \\
30 & 18 & False & False & mirrored & sobol & default & IPOP & csa & 20.000000 & 10.000000 & 0.300213 \\
30 & 19 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.283632 \\
30 & 19 & True & True & mirrored pairwise & sobol & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.282126 \\
30 & 19 & True & True & mirrored & sobol & equal & BIPOP & csa & 5.000000 & 5.000000 & 0.285517 \\
30 & 19 & True & True & mirrored & sobol & equal & BIPOP & csa & 5.000000 & 5.000000 & 0.288477 \\
30 & 19 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.284960 \\
30 & 20 & True & True & mirrored & sobol & default & BIPOP & csa & 5.000000 & 2.000000 & 0.177904 \\
30 & 20 & True & False & mirrored pairwise & sobol & default & IPOP & psr & 5.000000 & 2.000000 & 0.179476 \\
30 & 20 & True & False & mirrored pairwise & sobol & 1/2^lambda & IPOP & psr & 5.000000 & 2.000000 & 0.178383 \\
30 & 20 & True & True & mirrored & halton & equal & BIPOP & csa & 5.000000 & 2.000000 & 0.177080 \\
30 & 20 & False & False & mirrored & sobol & equal & BIPOP & psr & 5.000000 & 2.000000 & 0.179179 \\
30 & 21 & True & True & mirrored & gaussian & default & IPOP & csa & 14.000000 & 5.000000 & 0.848222 \\
30 & 21 & True & False & mirrored pairwise & halton & equal & BIPOP & psr & 10.000000 & 5.000000 & 0.662783 \\
30 & 21 & True & True & mirrored & halton & default & BIPOP & csa & 14.000000 & 10.000000 & 0.757834 \\
30 & 21 & False & False & mirrored & gaussian & 1/2^lambda & IPOP & csa & 5.000000 & 5.000000 & 0.898532 \\
30 & 21 & False & False & mirrored & gaussian & default & IPOP & psr & 14.000000 & 10.000000 & 0.877665 \\
30 & 22 & True & False & mirrored & halton & 1/2^lambda & BIPOP & psr & 10.000000 & 5.000000 & 0.432402 \\
30 & 22 & True & True & mirrored & gaussian & 1/2^lambda & BIPOP & csa & 5.000000 & 5.000000 & 0.344185 \\
30 & 22 & True & False & mirrored & sobol & default & BIPOP & psr & 5.000000 & 2.000000 & 0.308945 \\
30 & 22 & True & True & mirrored pairwise & sobol & 1/2^lambda & BIPOP & psr & 5.000000 & 2.000000 & 0.248296 \\
30 & 22 & False & False & mirrored pairwise & gaussian & 1/2^lambda & BIPOP & psr & 10.000000 & 10.000000 & 0.207998 \\
30 & 23 & True & False & mirrored pairwise & gaussian & default & IPOP & psr & 20.000000 & 5.000000 & 0.298122 \\
30 & 23 & False & False & mirrored & sobol & default & IPOP & psr & 20.000000 & 5.000000 & 0.298952 \\
30 & 23 & True & False & mirrored & gaussian & default & BIPOP & psr & 20.000000 & 20.000000 & 0.296533 \\
30 & 23 & False & False & mirrored pairwise & gaussian & default & BIPOP & psr & 20.000000 & 5.000000 & 0.294898 \\
30 & 23 & False & False & mirrored pairwise & sobol & default & BIPOP & psr & 20.000000 & 10.000000 & 0.285951 \\
30 & 24 & True & False & mirrored & sobol & default & IPOP & csa & 14.000000 & 4.000000 & 0.031490 \\
30 & 24 & False & False & mirrored & halton & equal & BIPOP & psr & 20.000000 & 5.000000 & 0.029699 \\
30 & 24 & False & False & mirrored & halton & equal & BIPOP & csa & 20.000000 & 10.000000 & 0.038790 \\
30 & 24 & False & False & mirrored & sobol & equal & IPOP & psr & 20.000000 & 5.000000 & 0.029582 \\
30 & 24 & False & False & mirrored & halton & equal & BIPOP & csa & 20.000000 & 10.000000 & 0.040257 \\
\bottomrule
\end{tabular}


==> hallOfFame/cma_es-hall-of-fame_BNW.tex <==
%\textcolor{blue}{bounds} - \textcolor{orange}{gaps/clusters} - \textcolor{red}{centre}

\begin{table}[ht]
\centering
\caption{Hall of fame of \textbf{modular CMA-ES}: best configurations per function including average best (denoted by All in fid), with resulting values of AOCC and structural BIAS indicator. Denoted in brackets after each module setting is the average effect in AOCC score of choosing the respective option versus all other choices (keeping the rest of the settings the same) \label{tab:fame-cma}}
\resizebox{\textwidth}{!}{\begin{tabular}{ccrrlllllrrrrl}
\toprule
\multicolumn{1}{c}{d} & \multicolumn{1}{c}{fid} & \multicolumn{1}{c}{active} & \multicolumn{1}{c}{base\_sampler} & \multicolumn{1}{c}{covariance} & \multicolumn{1}{c}{elitist} & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{local\_restart} & \multicolumn{1}{c}{mirrored} & \multicolumn{1}{c}{$\mu$} & \multicolumn{1}{c}{ssa} & \multicolumn{1}{c}{weights} & \multicolumn{1}{c}{AOCC} & \multicolumn{1}{c}{BIAS} \\
\midrule
5 & \textbf{All} & True (0.04) & gaussian (0.19) & True (0.13) & False (0.28) & 20 (0.38) & IPOP (0.02) & mirrored (0.05) & 10 (0.25) & csa (0.08) & default (0.09) & 0.666806 & \textcolor{red}{centre}\\
5 & 1 & False (0.00) & halton (0.00) & True (0.85) & True (0.00) & 5 (0.10) & BIPOP (0.00) & mirrored (0.00) & 5 (0.00) & csa (0.08) & $1/2^\lambda$ (0.16) & 0.983122 & \textcolor{red}{centre}\\
5 & 2 & True (0.03) & sobol (0.02) & False (0.01) & False (0.91) & 8 (0.20) & IPOP (0.00) & mirrored (0.04) & 5 (0.00) & csa (0.03) & $1/2^\lambda$ (0.46) & 0.907190 & \textcolor{red}{centre}\\
5 & 3 & True (0.11) & sobol (0.18) & True (0.19) & False (0.16) & 20 (0.27) & BIPOP (0.15) & pairwise (0.21) & 5 (0.30) & csa (0.19) & equal (0.19) & 0.378857 & \textcolor{red}{centre}\\
5 & 4 & False (0.00) & gaussian (0.04) & True (0.06) & False (0.05) & 10 (0.05) & BIPOP (0.04) & mirrored (0.04) & 10 (0.04) & csa (0.08) & $1/2^\lambda$ (0.10) & 0.168084 & \textcolor{red}{centre}\\
5 & 5 & True (0.00) & gaussian (0.00) & True (0.01) & False (0.00) & 5 (0.02) & IPOP (0.00) & mirrored (0.00) & 5 (0.00) & psr (0.00) & default (0.03) & 0.998051 & \textcolor{red}{centre}\\
5 & 6 & False (0.00) & halton (0.01) & True (0.92) & True (0.05) & 5 (0.00) & BIPOP (0.00) & pairwise (0.00) & 2 (0.02) & csa (0.11) & $1/2^\lambda$ (0.01) & 0.952707 & \textcolor{red}{centre}\\
5 & 7 & False (0.09) & halton (0.04) & True (0.71) & True (0.85) & 20 (0.14) & BIPOP (0.00) & pairwise (0.05) & 10 (0.06) & csa (0.04) & equal (0.16) & 0.951310 & \textcolor{red}{centre}\\
5 & 8 & True (0.02) & sobol (0.06) & True (0.01) & False (0.06) & 8 (0.20) & IPOP (0.00) & mirrored (0.04) & 5 (0.01) & csa (0.07) & $1/2^\lambda$ (0.27) & 0.909659 & \textcolor{red}{centre}\\
5 & 9 & False (0.02) & sobol (0.05) & False (0.06) & False (0.84) & 5 (0.00) & IPOP (0.01) & mirrored (0.04) & 2 (0.72) & csa (0.11) & default (0.06) & 0.915234 & \textcolor{red}{centre}\\
5 & 10 & False (0.00) & sobol (0.20) & True (0.04) & True (0.90) & 5 (0.30) & IPOP (0.00) & mirrored (0.02) & 5 (0.07) & psr (0.04) & equal (0.47) & 0.903269 & \textcolor{red}{centre}\\
5 & 11 & True (0.10) & sobol (0.38) & True (0.02) & False (0.63) & 20 (0.71) & IPOP (0.00) & mirrored (0.10) & 10 (0.47) & csa (0.02) & default (0.05) & 0.917868 & \textcolor{red}{centre}\\
5 & 12 & True (0.03) & halton (0.05) & False (0.08) & False (0.85) & 8 (0.23) & BIPOP (0.00) & mirrored (0.07) & 5 (0.01) & csa (0.06) & $1/2^\lambda$ (0.37) & 0.859747 & \textcolor{red}{centre} \\
5 & 13 & True (0.00) & sobol (0.22) & True (0.00) & True (0.90) & 5 (0.76) & IPOP (0.00) & mirrored (0.77) & 5 (0.64) & psr (0.15) & equal (0.47) & 0.895403 & \textcolor{red}{centre}\\
5 & 14 & False (0.30) & sobol (0.01) & True (0.77) & True (0.78) & 5 (0.13) & IPOP (0.00) & pairwise (0.01) & 5 (0.02) & csa (0.01) & equal (0.03) & 0.954450 & \textcolor{red}{centre}\\
5 & 15 & False (0.00) & halton (0.13) & True (0.08) & False (0.32) & 200 (0.00) & BIPOP (0.00) & mirrored (0.13) & 100 (0.29) & psr (0.05) & default (0.30) & 0.481335 & \textcolor{red}{centre}\\
5 & 16 & True (0.18) & sobol (0.11) & True (0.37) & False (0.38) & 20 (0.43) & BIPOP (0.08) & mirrored (0.12) & 5 (0.43) & csa (0.31) & default (0.22) & 0.809630 & \textcolor{red}{centre}\\
5 & 17 & False (0.03) & sobol (0.02) & True (0.02) & False (0.10) & 20 (0.45) & BIPOP (0.00) & mirrored (0.05) & 10 (0.19) & csa (0.08) & default (0.11) & 0.897028 & \textcolor{red}{centre}\\
5 & 18 & True (0.08) & sobol (0.15) & True (0.21) & False (0.37) & 20 (0.56) & BIPOP (0.15) & mirrored (0.23) & 5 (0.31) & psr (0.14) & default (0.31) & 0.818370 & \textcolor{red}{centre}\\
5 & 19 & True (0.13) & halton (0.11) & False (0.12) & False (0.14) & 20 (0.18) & IPOP (0.00) & pairwise (0.10) & 10 (0.12) & csa (0.12) & default (0.12) & 0.402468 & \textcolor{red}{centre}\\
5 & 20 & True (0.06) & sobol (0.10) & True (0.11) & False (0.16) & 200 (0.19) & BIPOP (0.00) & mirrored (0.06) & 20 (0.14) & psr (0.03) & default (0.15) & 0.356620 & \textcolor{red}{centre}\\
5 & 21 & False (0.47) & halton (0.50) & True (0.21) & True (0.34) & 10 (0.34) & IPOP (0.02) & pairwise (0.25) & 5 (0.37) & psr (0.19) & default (0.19) & 0.844145 & \textcolor{red}{centre}\\
5 & 22 & False (0.58) & halton (0.34) & True (0.43) & True (0.21) & 5 (0.28) & BIPOP (0.03) & pairwise (0.12) & 5 (0.17) & psr (0.03) & $1/2^\lambda$ (0.28) & 0.793936 & \textcolor{blue}{bounds}\\
5 & 23 & True (0.22) & halton (0.14) & True (0.18) & False (0.48) & 20 (0.42) & BIPOP (0.02) & mirrored (0.23) & 5 (0.42) & psr (0.22) & default (0.21) & 0.664302 & \textcolor{red}{centre}\\
5 & 24 & False (0.01) & sobol (0.01) & True (0.03) & False (0.04) & 10 (0.03) & IPOP (0.01) & mirrored (0.03) & 5 (0.04) & csa (0.03) & default (0.02) & 0.141390 & \textcolor{red}{centre}\\
\midrule

%\textcolor{red}{centre}
%\textcolor{orange}{gaps/clusters}

30 & \textbf{All} & True (0.01) & sobol (0.05) & False (0.00) & False (0.16) & 14 (0.00) & IPOP (0.01) & mirrored (0.02) & 7 (0.01) & csa (0.01) & default (0.01) & 0.496598 & \textcolor{red}{centre}\\
30 & 1 & False (0.00) & sobol (0.17) & False (0.01) & False (0.06) & 5 (0.18) & IPOP (0.00) & mirrored (0.02) & 5 (0.01) & psr (0.01) & $1/2^\lambda$ (0.34) & 0.945324 & \textcolor{red}{centre}\\
30 & 2 & True (0.00) & sobol (0.07) & False (0.01) & True (0.22) & 10 (0.08) & IPOP (0.00) & pairwise (0.00) & 10 (0.04) & psr (0.21) & equal (0.10) & 0.294408 & \textcolor{orange}{gaps/clusters}\\
30 & 3 & False (0.00) & sobol (0.04) & False (0.00) & False (0.07) & 20 (0.04) & BIPOP (0.00) & mirrored (0.01) & 10 (0.02) & csa (0.00) & default (0.01) & 0.396627 & \textcolor{orange}{gaps/clusters}\\
30 & 4 & False (0.00) & sobol (0.04) & False (0.00) & False (0.06) & 20 (0.03) & BIPOP (0.00) & mirrored (0.01) & 10 (0.01) & csa (0.01) & default (0.01) & 0.382659 & \textcolor{red}{centre}\\
30 & 5 & False (0.06) & sobol (0.26) & True (0.06) & True (0.01) & 5 (0.04) & IPOP (0.00) & mirrored (0.01) & 5 (0.01) & psr (0.58) & default (0.01) & 0.992649 & \textcolor{blue}{bounds}\\
30 & 6 & True (0.02) & sobol (0.14) & False (0.03) & False (0.38) & 14 (0.00) & BIPOP (0.00) & mirrored (0.06) & 7 (0.01) & csa (0.10) & default (0.07) & 0.583744 & \textcolor{red}{centre}\\
30 & 7 & True (0.00) & sobol (0.03) & False (0.01) & False (0.12) & 14 (0.02) & IPOP (0.01) & pairwise (0.00) & 5 (0.01) & csa (0.04) & default (0.01) & 0.447991 & \textcolor{red}{centre}\\
30 & 8 & True (0.01) & sobol (0.03) & False (0.01) & False (0.22) & 5 (0.03) & IPOP (0.01) & mirrored (0.01) & 5 (0.01) & csa (0.02) & $1/2^\lambda$ (0.13) & 0.409491 & discretization\\
30 & 9 & False (0.01) & sobol (0.01) & True (0.16) & True (0.06) & 5 (0.02) & IPOP (0.01) & mirrored (0.00) & 5 (0.01) & csa (0.00) & equal (0.07) & 0.409810 & \textcolor{red}{centre}\\
30 & 10 & True (0.00) & sobol (0.04) & False (0.01) & True (0.20) & 10 (0.07) & IPOP (0.00) & pairwise (0.00) & 10 (0.03) & psr (0.19) & equal (0.09) & 0.289573 & \textcolor{orange}{gaps/clusters}\\
30 & 11 & True (0.01) & sobol (0.02) & True (0.04) & False (0.05) & 14 (0.00) & BIPOP (0.00) & mirrored (0.03) & 7 (0.01) & psr (0.01) & default (0.01) & 0.408763 & \textcolor{red}{centre}\\
30 & 12 & False (0.03) & sobol (0.08) & True (0.51) & True (0.04) & 5 (0.17) & BIPOP (0.06) & mirrored (0.06) & 5 (0.05) & csa (0.11) & $1/2^\lambda$ (0.22) & 0.505465 & \textcolor{red}{centre}\\
30 & 13 & True (0.03) & sobol (0.06) & False (0.04) & False (0.07) & 14 (0.00) & BIPOP (0.03) & mirrored (0.04) & 7 (0.03) & psr (0.03) & default (0.05) & 0.511117 & \textcolor{red}{centre}\\
30 & 14 & False (0.00) & gaussian (0.03) & True (0.31) & True (0.02) & 5 (0.09) & BIPOP (0.00) & mirrored (0.01) & 5 (0.01) & csa (0.03) & $1/2^\lambda$ (0.14) & 0.704631 & \textcolor{red}{centre}\\
30 & 15 & True (0.00) & sobol (0.02) & False (0.01) & False (0.03) & 20 (0.04) & IPOP (0.00) & mirrored (0.01) & 10 (0.02) & psr (0.00) & default (0.01) & 0.398682 & \textcolor{red}{centre}\\
30 & 16 & True (0.00) & sobol (0.03) & False (0.01) & False (0.10) & 20 (0.06) & IPOP (0.01) & mirrored (0.04) & 10 (0.02) & csa (0.01) & default (0.03) & 0.499925 & \textcolor{red}{centre}\\
30 & 17 & True (0.00) & sobol (0.08) & False (0.02) & False (0.20) & 20 (0.10) & BIPOP (0.00) & mirrored (0.01) & 10 (0.03) & csa (0.02) & default (0.06) & 0.635100 & \textcolor{red}{centre}\\
30 & 18 & True (0.00) & sobol (0.07) & False (0.00) & False (0.15) & 20 (0.08) & BIPOP (0.00) & pairwise (0.02) & 10 (0.03) & csa (0.03) & default (0.02) & 0.549818 & \textcolor{red}{centre}\\
30 & 19 & True (0.00) & gaussian (0.01) & True (0.10) & True (0.03) & 5 (0.04) & BIPOP (0.09) & mirrored (0.00) & 5 (0.00) & csa (0.10) & equal (0.04) & 0.548607 & \textcolor{red}{centre}\\
30 & 20 & True (0.00) & sobol (0.01) & True (0.26) & True (0.00) & 5 (0.02) & IPOP (0.00) & mirrored (0.00) & 5 (0.00) & csa (0.00) & $1/2^\lambda$ (0.04) & 0.481448 & \textcolor{orange}{gaps/clusters}\\
30 & 21 & True (0.12) & sobol (0.16) & True (0.28) & True (0.18) & 14 (0.00) & IPOP (0.17) & mirrored (0.18) & 7 (0.12) & csa (0.15) & $1/2^\lambda$ (0.14) & 0.664094 & \textcolor{red}{centre}\\
30 & 22 & True (0.01) & gaussian (0.03) & True (0.10) & True (0.03) & 5 (0.04) & BIPOP (0.02) & mirrored (0.03) & 5 (0.01) & csa (0.04) & $1/2^\lambda$ (0.06) & 0.481261 & \textcolor{red}{centre}\\
30 & 23 & False (0.01) & sobol (0.02) & True (0.00) & False (0.09) & 20 (0.05) & IPOP (0.00) & pairwise (0.01) & 10 (0.01) & psr (0.09) & default (0.01) & 0.549599 & \textcolor{red}{centre}\\
30 & 24 & True (0.00) & sobol (0.01) & False (0.00) & False (0.03) & 20 (0.02) & IPOP (0.00) & mirrored (0.00) & 10 (0.01) & psr (0.01) & default (0.01) & 0.384299 & \textcolor{red}{centre}\\
% 5 & \textbf{All} & True (0.05) & halton (0.01) & True (0.11) & False (0.29) & 20 (0.42) & IPOP (0.03) & mirrored (0.02) & 10 (0.26) & csa (0.06) & default (0.08) & 0.676553 & \textcolor{red}{centre} \\
% 5 & 1 & False (0.00) & halton (0.00) & True (0.84) & True (0.01) & 5 (0.05) & BIPOP (0.00) & mirrored (0.00) & 5 (0.00) & csa (0.02) & $1/2^\lambda$ (0.45) & 0.984495 & \textcolor{orange}{gaps/clusters} \\
% 5 & 2 & True (0.03) & sobol (0.02) & False (0.01) & False (0.91) & 8 (0.11) & IPOP (0.00) & mirrored (0.02) & 5 (0.00) & csa (0.03) & $1/2^\lambda$ (0.46) & 0.907190 & \textcolor{orange}{gaps/clusters} \\
% 5 & 3 & True (0.33) & halton (0.29) & False (0.31) & False (0.43) & 8 (0.00) & BIPOP (0.00) & mirrored (0.35) & 3 (0.23) & csa (0.37) & default (0.34) & 0.472781 & \textcolor{red}{centre} \\
% 5 & 4 & False (0.17) & halton (0.17) & True (0.26) & True (0.16) & 8 (0.00) & IPOP (0.02) & pairwise (0.17) & 3 (0.11) & csa (0.19) & $1/2^\lambda$ (0.17) & 0.287226 & \textcolor{red}{centre} \\
% 5 & 5 & True (0.00) & gaussian (0.00) & True (0.01) & False (0.00) & 5 (0.01) & IPOP (0.00) & mirrored (0.00) & 5 (0.00) & psr (0.00) & default (0.03) & 0.998051  & - \\
% 5 & 6 & True (0.01) & halton (0.02) & True (0.91) & True (0.18) & 5 (0.12) & BIPOP (0.00) & pairwise (0.89) & 5 (0.01) & csa (0.16) & default (0.69) & 0.953062 & \textcolor{orange}{gaps/clusters} \\
% 5 & 7 & True (0.15) & halton (0.37) & False (0.00) & False (0.77) & 20 (0.68) & BIPOP (0.00) & mirrored (0.28) & 10 (0.43) & psr (0.28) & default (0.22) & 0.962005 & - \\
% 5 & 8 & True (0.07) & halton (0.09) & True (0.92) & True (0.09) & 8 (0.28) & BIPOP (0.00) & pairwise (0.11) & 5 (0.07) & csa (0.36) & default (0.42) & 0.922699 & \textcolor{orange}{gaps/clusters} \\
% 5 & 9 & False (0.02) & sobol (0.03) & False (0.06) & False (0.84) & 5 (0.00) & IPOP (0.03) & mirrored (0.03) & 2 (0.72) & csa (0.11) & default (0.06) & 0.915234 & \textcolor{orange}{gaps/clusters} \\
% 5 & 10 & False (0.00) & halton (0.01) & True (0.02) & True (0.91) & 5 (0.17) & BIPOP (0.00) & mirrored (0.01) & 5 (0.08) & psr (0.06) & equal (0.47) & 0.906337 & - \\
% 5 & 11 & True (0.10) & sobol (0.01) & True (0.02) & False (0.63) & 20 (0.77) & IPOP (0.00) & mirrored (0.05) & 10 (0.47) & csa (0.02) & default (0.05) & 0.917868 & \textcolor{red}{centre} \\
% 5 & 12 & True (0.06) & halton (0.04) & False (0.02) & False (0.87) & 8 (0.00) & BIPOP (0.00) & mirrored (0.08) & 3 (0.02) & csa (0.13) & default (0.16) & 0.870508 & \textcolor{red}{centre} \\
% 5 & 13 & False (0.00) & halton (0.02) & True (0.02) & True (0.91) & 5 (0.20) & BIPOP (0.00) & mirrored (0.02) & 5 (0.32) & psr (0.14) & equal (0.48) & 0.905252 & - \\
% 5 & 14 & False (0.30) & sobol (0.01) & True (0.77) & True (0.78) & 5 (0.07) & IPOP (0.00) & pairwise (0.01) & 5 (0.02) & csa (0.01) & equal (0.03) & 0.954450 & \textcolor{red}{centre} \\
% 5 & 15 & True (0.29) & halton (0.10) & True (0.33) & False (0.35) & 20 (0.35) & IPOP (0.12) & mirrored (0.15) & 10 (0.31) & csa (0.32) & default (0.27) & 0.492284 & \textcolor{red}{centre} \\
% 5 & 16 & True (0.13) & halton (0.14) & True (0.06) & False (0.29) & 20 (0.44) & BIPOP (0.04) & mirrored (0.13) & 5 (0.31) & csa (0.49) & default (0.42) & 0.866222 & \textcolor{red}{centre} \\
% 5 & 17 & False (0.01) & halton (0.02) & True (0.05) & False (0.11) & 20 (0.51) & BIPOP (0.00) & mirrored (0.03) & 10 (0.19) & csa (0.07) & default (0.13) & 0.904906 & \textcolor{red}{centre} \\
% 5 & 18 & True (0.15) & halton (0.14) & True (0.22) & False (0.41) & 20 (0.56) & BIPOP (0.00) & mirrored (0.31) & 5 (0.21) & psr (0.09) & default (0.45) & 0.850612 & - \\
% 5 & 19 & False (0.16) & halton (0.15) & True (0.16) & False (0.10) & 20 (0.10) & BIPOP (0.03) & mirrored (0.16) & 5 (0.16) & csa (0.17) & $1/2^\lambda$ (0.11) & 0.412441 & discretisation \\
% 5 & 20 & False (0.24) & halton (0.26) & True (0.30) & True (0.27) & 8 (0.22) & IPOP (0.15) & pairwise (0.26) & 5 (0.16) & csa (0.27) & default (0.28) & 0.463041 & \textcolor{red}{centre} \\
% 5 & 21 & False (0.21) & halton (0.31) & True (0.84) & True (0.26) & 5 (0.00) & IPOP (0.16) & mirrored (0.32) & 2 (0.84) & csa (0.66) & default (0.30) & 0.951148 & \textcolor{red}{centre} \\
% 5 & 22 & True (0.11) & halton (0.14) & True (0.75) & True (0.46) & 5 (0.00) & IPOP (0.21) & pairwise (0.30) & 2 (0.16) & csa (0.52) & $1/2^\lambda$ (0.21) & 0.812444 & \textcolor{red}{centre} \\
% 5 & 23 & False (0.23) & halton (0.37) & False (0.22) & False (0.51) & 20 (0.44) & BIPOP (0.00) & mirrored (0.32) & 5 (0.28) & psr (0.44) & default (0.32) & 0.674847 & - \\
% 5 & 24 & False (0.00) & halton (0.02) & True (0.01) & False (0.03) & 8 (0.00) & IPOP (0.02) & mirrored (0.01) & 3 (0.02) & csa (0.04) & $1/2^\lambda$ (0.02) & 0.141660 & \textcolor{orange}{gaps/clusters} \\ 
% \midrule
% 30 & \textbf{All} & True (0.01) & sobol (0.05) & False (0.00) & False (0.16) & 14 (0.00) & IPOP (0.00) & mirrored (0.01) & 4 (0.01) & csa (0.01) & default (0.01) & 0.496598 & \textcolor{orange}{gaps/clusters} \\
% 30 & 1 & False (0.00) & sobol (0.12) & False (0.01) & False (0.06) & 5 (0.11) & IPOP (0.00) & mirrored (0.01) & 5 (0.01) & psr (0.01) & $1/2^\lambda$ (0.34) & 0.945324 & - \\
% 30 & 2 & True (0.00) & sobol (0.06) & False (0.01) & True (0.22) & 10 (0.07) & IPOP (0.00) & pairwise (0.01) & 10 (0.04) & psr (0.21) & equal (0.10) & 0.294408 & - \\
% 30 & 3 & False (0.00) & sobol (0.04) & False (0.00) & False (0.07) & 20 (0.04) & BIPOP (0.00) & mirrored (0.01) & 10 (0.02) & csa (0.00) & default (0.01) & 0.396627 & \textcolor{red}{centre} \\
% 30 & 4 & False (0.00) & sobol (0.04) & False (0.00) & False (0.06) & 20 (0.03) & BIPOP (0.00) & mirrored (0.00) & 10 (0.01) & csa (0.01) & default (0.01) & 0.382659 & \textcolor{orange}{gaps/clusters} \\
% 30 & 5 & False (0.06) & sobol (0.02) & True (0.06) & True (0.01) & 5 (0.03) & IPOP (0.00) & mirrored (0.01) & 5 (0.01) & psr (0.58) & default (0.01) & 0.992649  & - \\
% 30 & 6 & True (0.02) & sobol (0.14) & False (0.03) & False (0.38) & 14 (0.00) & BIPOP (0.00) & mirrored (0.03) & 4 (0.01) & csa (0.10) & default (0.07) & 0.583744 & \textcolor{orange}{gaps/clusters} \\
% 30 & 7 & True (0.00) & sobol (0.04) & False (0.01) & False (0.12) & 14 (0.02) & IPOP (0.01) & pairwise (0.00) & 5 (0.00) & csa (0.04) & default (0.01) & 0.447991 & \textcolor{orange}{gaps/clusters} \\
% 30 & 8 & True (0.01) & sobol (0.01) & False (0.01) & False (0.22) & 5 (0.02) & IPOP (0.01) & mirrored (0.01) & 5 (0.01) & csa (0.02) & $1/2^\lambda$ (0.13) & 0.409491 & discretisation \\
% 30 & 9 & False (0.01) & sobol (0.02) & True (0.16) & True (0.06) & 5 (0.01) & IPOP (0.01) & mirrored (0.00) & 5 (0.01) & csa (0.00) & equal (0.07) & 0.409810 & \textcolor{orange}{gaps/clusters} \\
% 30 & 10 & True (0.00) & sobol (0.03) & False (0.01) & True (0.20) & 10 (0.06) & IPOP (0.00) & pairwise (0.00) & 10 (0.03) & psr (0.19) & equal (0.09) & 0.289573  & - \\
% 30 & 11 & True (0.01) & sobol (0.03) & True (0.04) & False (0.05) & 14 (0.00) & BIPOP (0.00) & mirrored (0.02) & 4 (0.00) & psr (0.01) & default (0.01) & 0.408763  & - \\
% 30 & 12 & False (0.03) & sobol (0.11) & True (0.51) & True (0.04) & 5 (0.13) & BIPOP (0.05) & mirrored (0.05) & 5 (0.05) & csa (0.11) & $1/2^\lambda$ (0.22) & 0.505465 & \textcolor{orange}{gaps/clusters} \\
% 30 & 13 & True (0.03) & sobol (0.06) & False (0.04) & False (0.07) & 14 (0.00) & BIPOP (0.03) & mirrored (0.04) & 4 (0.02) & psr (0.03) & default (0.05) & 0.511117 & - \\
% 30 & 14 & False (0.00) & gaussian (0.03) & True (0.31) & True (0.02) & 5 (0.06) & BIPOP (0.00) & mirrored (0.01) & 5 (0.01) & csa (0.03) & $1/2^\lambda$ (0.14) & 0.704631 & \textcolor{orange}{gaps/clusters} \\
% 30 & 15 & True (0.00) & sobol (0.01) & False (0.01) & False (0.03) & 20 (0.04) & IPOP (0.00) & mirrored (0.01) & 10 (0.02) & psr (0.00) & default (0.01) & 0.398682 & - \\
% 30 & 16 & True (0.00) & sobol (0.03) & False (0.01) & False (0.10) & 20 (0.06) & IPOP (0.00) & mirrored (0.02) & 10 (0.02) & csa (0.01) & default (0.03) & 0.499925 & \textcolor{red}{centre} \\
% 30 & 17 & True (0.00) & sobol (0.08) & False (0.02) & False (0.20) & 20 (0.11) & BIPOP (0.00) & mirrored (0.01) & 10 (0.03) & csa (0.02) & default (0.06) & 0.635100 & \textcolor{red}{centre} \\
% 30 & 18 & True (0.00) & sobol (0.07) & False (0.00) & False (0.15) & 20 (0.09) & BIPOP (0.00) & pairwise (0.01) & 10 (0.03) & csa (0.03) & default (0.02) & 0.549818 & \textcolor{orange}{gaps/clusters} \\
% 30 & 19 & True (0.00) & gaussian (0.01) & True (0.10) & True (0.03) & 5 (0.03) & BIPOP (0.09) & mirrored (0.01) & 5 (0.00) & csa (0.10) & equal (0.04) & 0.548607 & \textcolor{orange}{gaps/clusters} \\
% 30 & 20 & True (0.00) & sobol (0.01) & True (0.26) & True (0.00) & 5 (0.01) & IPOP (0.00) & mirrored (0.00) & 5 (0.00) & csa (0.00) & $1/2^\lambda$ (0.04) & 0.481448 & \textcolor{orange}{gaps/clusters} \\
% 30 & 21 & True (0.12) & sobol (0.17) & True (0.28) & True (0.18) & 14 (0.00) & IPOP (0.19) & mirrored (0.15) & 4 (0.09) & csa (0.15) & $1/2^\lambda$ (0.14) & 0.664094 & \textcolor{orange}{gaps/clusters} \\
% 30 & 22 & False (0.05) & halton (0.04) & True (0.05) & False (0.05) & 10 (0.05) & BIPOP (0.00) & mirrored (0.06) & 5 (0.05) & psr (0.06) & $1/2^\lambda$ (0.05) & 0.485074 & - \\
% 30 & 23 & False (0.01) & sobol (0.01) & True (0.00) & False (0.09) & 20 (0.05) & IPOP (0.00) & pairwise (0.01) & 10 (0.01) & psr (0.09) & default (0.01) & 0.549599 & - \\
% 30 & 24 & True (0.00) & sobol (0.01) & False (0.00) & False (0.03) & 20 (0.03) & IPOP (0.00) & mirrored (0.00) & 10 (0.01) & psr (0.01) & default (0.01) & 0.384299 & - \\

% \toprule
% dim & fid & active & cov. & elitist & mirrored & sampler & weights & local restart & sza & $\lambda$ & $\mu$ & AOCC & BIAS \\
% \midrule


\bottomrule
\end{tabular}}
\end{table} 


==> hallOfFame/de-hall-of-fame_BNW.tex <==
%\textcolor{blue}{bounds} - \textcolor{orange}{gaps/clusters} - \textcolor{red}{centre}

\begin{table}[ht]
\caption{Hall of fame of \textbf{modular DE}: best configurations per function including average best (denoted by All in fid), with resulting values of AOCC and structural BIAS indicator. Denoted in brackets after each module setting is the average effect in AOCC score of choosing the respective option versus all other choices (keeping the rest of the settings the same). \label{tab:fame-de} }
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ccrrrllrrllrrrl}
\toprule
\multicolumn{1}{c}{d} & \multicolumn{1}{c}{fid} & \multicolumn{1}{c}{CR} & \multicolumn{1}{c}{F} & \multicolumn{1}{c}{adaptation} & \multicolumn{1}{c}{crossover} & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{lpsr} & \multicolumn{1}{c}{base} & \multicolumn{1}{c}{diffs} & \multicolumn{1}{c}{ref} & \multicolumn{1}{c}{archive} & \multicolumn{1}{c}{AOCC} & \multicolumn{1}{c}{BIAS} \\
\midrule
5 & \textbf{All} & 0.75 (0.09) & 0.5 (0.09) & shade (0.06) & exp (0.05) & 10 (0.18) & False (0.02) & target (0.16) & 2 (0.08) & pbest (0.05) & True (0.10) & 0.566908 & \textcolor{blue}{bounds} \\
5 & 1 & 0.25 (0.25) & 0.25 (0.29) & nan (0.12) & bin (0.01) & 8 (0.06) & False (0.19) & best (0.34) & 1 (0.00) & rand (0.02) & True (0.55) & 0.971233 & \textcolor{orange}{gaps/clusters} \\
5 & 2 & 0.25 (0.37) & 0.25 (0.45) & nan (0.14) & bin (0.01) & 8 (0.13) & False (0.38) & best (0.31) & 2 (0.00) & rand (0.01) & True (0.11) & 0.940875  & \textcolor{blue}{bounds} \\
5 & 3 & 0.05 (0.40) & 0.5 (0.59) & nan (0.13) & exp (0.00) & 8 (0.33) & False (0.59) & target (0.10) & 2 (0.18) & rand (0.08) & True (0.06) & 0.885237 & - \\
5 & 4 & 0.05 (0.38) & 0.5 (0.17) & shade (0.26) & exp (0.16) & 8 (0.35) & False (0.59) & rand (0.30) & 1 (0.35) & best (0.28) & True (0.41) & 0.816036 & \textcolor{blue}{bounds} \\
5 & 5 & 0.75 (0.11) & 1.25 (0.02) & shade (0.03) & bin (0.06) & 8 (0.03) & False (0.01) & best (0.12) & 1 (0.06) & best (0.14) & True (0.18) & 0.997461 & \textcolor{blue}{bounds} \\
5 & 6 & 0.75 (0.07) & 0.25 (0.42) & shade (0.35) & bin (0.01) & 10 (0.33) & True (0.00) & target (0.36) & 2 (0.05) & best (0.09) & True (0.05) & 0.878111 & \textcolor{orange}{gaps/clusters} \\
5 & 7 & 1.0 (0.35) & 0.5 (0.44) & nan (0.08) & bin (0.09) & 50 (0.78) & False (0.04) & target (0.18) & 1 (0.24) & pbest (0.33) & False (0.17) & 0.909025 & \textcolor{orange}{gaps/clusters} \\
5 & 8 & 1.0 (0.20) & 0.5 (0.27) & shade (0.35) & bin (0.33) & 10 (0.35) & True (0.04) & target (0.20) & 1 (0.27) & pbest (0.18) & True (0.71) & 0.814825 & \textcolor{blue}{bounds} \\
5 & 9 & 0.75 (0.53) & 0.5 (0.51) & nan (0.06) & exp (0.01) & 10 (0.43) & True (0.01) & target (0.29) & 1 (0.09) & pbest (0.16) & True (0.66) & 0.799625 & - \\
5 & 10 & 1.0 (0.60) & 0.25 (0.56) & nan (0.30) & exp (0.04) & 10 (0.49) & True (0.01) & target (0.76) & 2 (0.25) & nan (0.74) & True (0.39) & 0.777871 & - \\
5 & 11 & 1.0 (0.57) & 0.25 (0.54) & nan (0.27) & exp (0.01) & 10 (0.42) & True (0.01) & target (0.76) & 2 (0.17) & nan (0.69) & True (0.26) & 0.832987 & - \\
5 & 12 & 1.0 (0.17) & 0.25 (0.27) & shade (0.36) & exp (0.15) & 10 (0.22) & False (0.06) & target (0.30) & 2 (0.21) & best (0.12) & True (0.19) & 0.547322 & - \\
5 & 13 & 1.0 (0.49) & 0.75 (0.55) & nan (0.20) & bin (0.00) & 50 (0.44) & True (0.08) & target (0.47) & 1 (0.33) & best (0.24) & False (0.51) & 0.714799 & \textcolor{blue}{bounds} \\
5 & 14 & 1.0 (0.10) & 0.5 (0.22) & shade (0.09) & bin (0.01) & 10 (0.22) & False (0.03) & target (0.29) & 2 (0.08) & pbest (0.08) & True (0.17) & 0.899397 & \textcolor{blue}{bounds} \\
5 & 15 & 0.05 (0.10) & 0.25 (0.09) & jDE (0.14) & exp (0.11) & 8 (0.13) & False (0.15) & target (0.13) & 2 (0.09) & pbest (0.11) & True (0.11) & 0.246889 & \textcolor{blue}{bounds} \\
5 & 16 & 1.0 (0.30) & 0.25 (0.32) & nan (0.25) & exp (0.08) & 8 (0.22) & True (0.29) & best (0.33) & 2 (0.10) & rand (0.14) & True (0.09) & 0.466607 & \textcolor{blue}{bounds} \\
5 & 17 & 1.0 (0.33) & 0.5 (0.34) & nan (0.16) & exp (0.03) & 50 (0.31) & True (0.03) & target (0.24) & 1 (0.29) & pbest (0.25) & False (0.26) & 0.713114 & \textcolor{red}{centre} \\
5 & 18 & 1.0 (0.33) & 0.5 (0.35) & nan (0.19) & bin (0.01) & 50 (0.31) & True (0.02) & target (0.25) & 1 (0.30) & pbest (0.29) & False (0.25) & 0.664711 & \textcolor{red}{centre} \\
5 & 19 & 0.75 (0.04) & 0.25 (0.05) & jDE (0.06) & exp (0.05) & 10 (0.05) & False (0.03) & best (0.05) & 1 (0.04) & nan (0.05) & True (0.09) & 0.259360 & \textcolor{blue}{bounds} \\
5 & 20 & 0.25 (0.25) & 0.5 (0.26) & shade (0.22) & exp (0.13) & 10 (0.37) & True (0.16) & rand (0.29) & 1 (0.11) & nan (0.21) & True (0.37) & 0.678659 & \textcolor{blue}{bounds} \\
5 & 21 & 1.0 (0.18) & 0.25 (0.26) & shade (0.16) & exp (0.07) & 50 (0.35) & True (0.07) & target (0.27) & 1 (0.10) & pbest (0.23) & False (0.02) & 0.725264 & \textcolor{red}{centre} \\
5 & 22 & 0.75 (0.19) & 0.25 (0.33) & shade (0.15) & bin (0.17) & 50 (0.38) & True (0.10) & target (0.39) & 1 (0.16) & best (0.23) & False (0.12) & 0.724567 & \textcolor{red}{centre} \\
5 & 23 & 0.75 (0.04) & 0.25 (0.05) & shade (0.05) & exp (0.04) & 50 (0.06) & True (0.04) & best (0.05) & 2 (0.03) & nan (0.05) & False (0.04) & 0.236681 & \textcolor{blue}{bounds} \\
5 & 24 & 1.0 (0.03) & 0.5 (0.05) & nan (0.02) & bin (0.01) & 50 (0.03) & True (0.00) & target (0.04) & 1 (0.05) & best (0.02) & False (0.04) & 0.123116 & \textcolor{orange}{gaps/clusters} \\
\midrule
30 & \textbf{All} & 0.25 (0.03) & 0.5 (0.02) & shade (0.02) & bin (0.04) & 14 (0.10) & False (0.07) & target (0.04) & 1 (0.01) & pbest (0.02) & True (0.02) & 0.443169  & - \\
30 & 1 & 0.25 (0.13) & 0.5 (0.10) & shade (0.04) & bin (0.16) & 14 (0.34) & False (0.27) & target (0.20) & 1 (0.04) & pbest (0.10) & True (0.10) & 0.786120  & - \\
30 & 2 & 0.25 (0.22) & 0.75 (0.38) & nan (0.19) & bin (0.19) & 14 (0.38) & False (0.32) & target (0.32) & 1 (0.24) & pbest (0.13) & False (0.14) & 0.565194  & - \\
30 & 3 & 0.05 (0.02) & 0.5 (0.01) & shade (0.01) & exp (0.02) & 14 (0.09) & False (0.08) & rand (0.03) & 1 (0.02) & nan (0.03) & True (0.00) & 0.422156  & - \\
30 & 4 & 0.05 (0.02) & 0.5 (0.01) & shade (0.01) & exp (0.01) & 14 (0.08) & False (0.07) & rand (0.03) & 1 (0.02) & nan (0.02) & True (0.00) & 0.405671  & - \\
30 & 5 & 0.25 (0.32) & 1.75 (0.03) & nan (0.29) & bin (0.05) & 14 (0.23) & False (0.11) & best (0.02) & 2 (0.14) & best (0.02) & True (0.03) & 0.970231 & \textcolor{blue}{bounds} \\
30 & 6 & 0.05 (0.01) & 0.75 (0.00) & jDE (0.05) & bin (0.04) & 14 (0.12) & False (0.07) & target (0.04) & 2 (0.01) & rand (0.02) & True (0.03) & 0.382355 & \textcolor{orange}{gaps/clusters} \\
30 & 7 & 0.75 (0.03) & 0.5 (0.06) & nan (0.01) & bin (0.04) & 60 (0.03) & True (0.01) & target (0.06) & 1 (0.04) & pbest (0.03) & True (0.01) & 0.416182 & - \\
30 & 8 & 0.25 (0.06) & 0.5 (0.12) & nan (0.01) & bin (0.04) & 14 (0.13) & False (0.10) & target (0.07) & 2 (0.01) & pbest (0.03) & True (0.02) & 0.375220 & - \\
30 & 9 & 0.75 (0.00) & 0.5 (0.01) & jDE (0.02) & bin (0.02) & 14 (0.09) & False (0.05) & target (0.03) & 1 (0.01) & pbest (0.02) & True (0.04) & 0.382241 & - \\
30 & 10 & 1.0 (0.06) & 0.25 (0.06) & shade (0.03) & bin (0.01) & 14 (0.02) & True (0.02) & target (0.04) & 2 (0.01) & pbest (0.03) & True (0.02) & 0.224865 & \textcolor{orange}{gaps/clusters} \\
30 & 11 & 1.0 (0.04) & 0.25 (0.05) & nan (0.02) & exp (0.00) & 14 (0.01) & True (0.03) & target (0.03) & 2 (0.01) & pbest (0.02) & True (0.01) & 0.392524 & \textcolor{red}{centre} \\
30 & 12 & 0.25 (0.12) & 0.5 (0.08) & shade (0.03) & bin (0.17) & 14 (0.28) & False (0.22) & target (0.15) & 1 (0.03) & pbest (0.08) & True (0.10) & 0.340692 & - \\
30 & 13 & 0.25 (0.04) & 0.5 (0.03) & shade (0.03) & bin (0.06) & 14 (0.09) & False (0.07) & target (0.06) & 1 (0.00) & pbest (0.03) & True (0.05) & 0.418056 & - \\
30 & 14 & 0.5 (0.05) & 0.5 (0.08) & shade (0.03) & bin (0.05) & 14 (0.12) & False (0.08) & target (0.12) & 1 (0.01) & pbest (0.04) & True (0.08) & 0.595350 & - \\
30 & 15 & 0.75 (0.01) & 0.25 (0.01) & shade (0.01) & bin (0.01) & 14 (0.03) & False (0.02) & rand (0.02) & 2 (0.00) & rand (0.00) & False (0.00) & 0.356576 & \textcolor{blue}{bounds} \\
30 & 16 & 0.75 (0.02) & 0.25 (0.03) & nan (0.01) & bin (0.02) & 14 (0.02) & False (0.02) & best (0.03) & 2 (0.01) & nan (0.00) & True (0.01) & 0.433995 & \textcolor{blue}{bounds} \\
30 & 17 & 0.5 (0.03) & 0.5 (0.05) & nan (0.01) & bin (0.05) & 60 (0.02) & True (0.01) & target (0.04) & 1 (0.04) & pbest (0.03) & False (0.00) & 0.497815 & - \\
30 & 18 & 0.75 (0.03) & 0.5 (0.04) & nan (0.01) & bin (0.04) & 60 (0.01) & True (0.01) & target (0.04) & 1 (0.03) & pbest (0.03) & False (0.01) & 0.459689 & \textcolor{red}{centre} \\
30 & 19 & 1.0 (0.01) & 0.25 (0.02) & shade (0.01) & bin (0.01) & 14 (0.01) & False (0.01) & target (0.01) & 1 (0.01) & best (0.01) & False (0.01) & 0.459233 & \textcolor{red}{centre} \\
30 & 20 & 0.25 (0.10) & 0.25 (0.21) & nan (0.02) & bin (0.02) & 14 (0.14) & False (0.08) & best (0.02) & 2 (0.01) & rand (0.02) & False (0.00) & 0.472318 & - \\
30 & 21 & 0.5 (0.05) & 0.25 (0.05) & shade (0.05) & bin (0.09) & 60 (0.07) & True (0.02) & target (0.06) & 1 (0.03) & best (0.07) & True (0.05) & 0.503991 & \textcolor{red}{centre} \\
30 & 22 & 0.05 (0.02) & 1.75 (0.02) & jDE (0.04) & bin (0.02) & 14 (0.04) & False (0.03) & target (0.03) & 1 (0.01) & best (0.02) & True (0.02) & 0.460824 & - \\
30 & 23 & 1.0 (0.01) & 0.25 (0.01) & shade (0.02) & exp (0.01) & 14 (0.02) & False (0.02) & best (0.02) & 2 (0.01) & nan (0.01) & True (0.03) & 0.481032 & \textcolor{blue}{bounds} \\
30 & 24 & 0.75 (0.01) & 0.5 (0.01) & shade (0.01) & exp (0.01) & 14 (0.02) & False (0.02) & best (0.01) & 1 (0.00) & rand (0.01) & False (0.00) & 0.352221 & \textcolor{blue}{bounds} \\

% \toprule
% dim & fid & F & CR & $\lambda$ & mu. base & mu. ref. & mu. comp. & archive & crossover & adapt. & lpsr & AOCC & BIAS \\
% \midrule
% 5 & All & 0.50 & 0.75 & 10 & target & pbest & 2 & True & exp & shade & False & 0.566908 & \textcolor{blue}{bounds} \\
% 5 & 1 & 0.25 & 0.25 & 8 & best & rand & 1 & True & bin & nan & False & 0.971233 & \textcolor{orange}{gaps/clusters} \\
% 5 & 2 & 0.25 & 0.25 & 8 & best & rand & 2 & True & bin & nan & False & 0.940875 & \textcolor{blue}{bounds} \\
% 5 & 3 & 0.50 & 0.05 & 8 & target & rand & 2 & True & exp & nan & False & 0.885237 & - \\
% 5 & 4 & 0.50 & 0.05 & 8 & rand & best & 1 & True & exp & shade & False & 0.816036 & \textcolor{blue}{bounds} \\
% 5 & 5 & 1.25 & 0.75 & 8 & best & best & 1 & True & bin & shade & False & 0.997461 & \textcolor{blue}{bounds} \\
% 5 & 6 & 0.25 & 0.75 & 10 & target & best & 2 & True & bin & shade & True & 0.878111 & \textcolor{orange}{gaps/clusters} \\
% 5 & 7 & 0.50 & 1.00 & 50 & target & pbest & 1 & False & bin & nan & False & 0.909025 & \textcolor{orange}{gaps/clusters} \\
% 5 & 8 & 0.50 & 1.00 & 10 & target & pbest & 1 & True & bin & shade & True & 0.814825 & \textcolor{blue}{bounds} \\
% 5 & 9 & 0.50 & 0.75 & 10 & target & pbest & 1 & True & exp & nan & True & 0.799625 & - \\
% 5 & 10 & 0.25 & 1.00 & 10 & target & nan & 2 & True & exp & nan & True & 0.777871 & - \\
% 5 & 11 & 0.25 & 1.00 & 10 & target & nan & 2 & True & exp & nan & True & 0.832987 & - \\
% 5 & 12 & 0.25 & 1.00 & 10 & target & best & 2 & True & exp & shade & False & 0.547322 & - \\
% 5 & 13 & 0.75 & 1.00 & 50 & target & best & 1 & False & bin & nan & True & 0.714799 & \textcolor{blue}{bounds} \\
% 5 & 14 & 0.50 & 1.00 & 10 & target & pbest & 2 & True & bin & shade & False & 0.899397 & \textcolor{blue}{bounds} \\
% 5 & 15 & 0.25 & 0.05 & 8 & target & pbest & 2 & True & exp & jDE & False & 0.246889 & \textcolor{blue}{bounds} \\
% 5 & 16 & 0.25 & 1.00 & 8 & best & rand & 2 & True & exp & nan & True & 0.466607 & \textcolor{blue}{bounds} \\
% 5 & 17 & 0.50 & 1.00 & 50 & target & pbest & 1 & False & exp & nan & True & 0.713114 & \textcolor{red}{centre} \\
% 5 & 18 & 0.50 & 1.00 & 50 & target & pbest & 1 & False & bin & nan & True & 0.664711 & \textcolor{red}{centre} \\
% 5 & 19 & 0.25 & 0.75 & 10 & best & nan & 1 & True & exp & jDE & False & 0.259360 & \textcolor{blue}{bounds} \\
% 5 & 20 & 0.50 & 0.25 & 10 & rand & nan & 1 & True & exp & shade & True & 0.678659 & \textcolor{blue}{bounds} \\
% 5 & 21 & 0.25 & 1.00 & 50 & target & pbest & 1 & False & exp & shade & True & 0.725264 & \textcolor{red}{centre} \\
% 5 & 22 & 0.25 & 0.75 & 50 & target & best & 1 & False & bin & shade & True & 0.724567 & \textcolor{red}{centre} \\
% 5 & 23 & 0.25 & 0.75 & 50 & best & nan & 2 & False & exp & shade & True & 0.236681 & \textcolor{blue}{bounds} \\
% 5 & 24 & 0.50 & 1.00 & 50 & target & best & 1 & False & bin & nan & True & 0.123116 & \textcolor{orange}{gaps/clusters} \\
% 30 & \textbf{All} & 0.50 & 0.25 & 14 & target & pbest & 1 & True & bin & shade & False & 0.443169 & - \\
% 30 & 1 & 0.50 & 0.25 & 14 & target & pbest & 1 & True & bin & shade & False & 0.786120 & - \\
% 30 & 2 & 0.75 & 0.25 & 14 & target & pbest & 1 & False & bin & nan & False & 0.565194 & - \\
% 30 & 3 & 0.50 & 0.05 & 14 & rand & nan & 1 & True & exp & shade & False & 0.422156 & - \\
% 30 & 4 & 0.50 & 0.05 & 14 & rand & nan & 1 & True & exp & shade & False & 0.405671 & - \\
% 30 & 5 & 1.75 & 0.25 & 14 & best & best & 2 & True & bin & nan & False & 0.970231 & \textcolor{blue}{bounds} \\
% 30 & 6 & 0.75 & 0.05 & 14 & target & rand & 2 & True & bin & jDE & False & 0.382355 & \textcolor{orange}{gaps/clusters} \\
% 30 & 7 & 0.50 & 0.75 & 60 & target & pbest & 1 & True & bin & nan & True & 0.416182 & - \\
% 30 & 8 & 0.50 & 0.25 & 14 & target & pbest & 2 & True & bin & nan & False & 0.375220 & - \\
% 30 & 9 & 0.50 & 0.75 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.382241 & - \\
% 30 & 10 & 0.25 & 1.00 & 14 & target & pbest & 2 & True & bin & shade & True & 0.224865 & \textcolor{orange}{gaps/clusters} \\
% 30 & 11 & 0.25 & 1.00 & 14 & target & pbest & 2 & True & exp & nan & True & 0.392524 & \textcolor{red}{centre} \\
% 30 & 12 & 0.50 & 0.25 & 14 & target & pbest & 1 & True & bin & shade & False & 0.340692 & - \\
% 30 & 13 & 0.50 & 0.25 & 14 & target & pbest & 1 & True & bin & shade & False & 0.418056 & - \\
% 30 & 14 & 0.50 & 0.50 & 14 & target & pbest & 1 & True & bin & shade & False & 0.595350 & - \\
% 30 & 15 & 0.25 & 0.75 & 14 & rand & rand & 2 & False & bin & shade & False & 0.356576 & \textcolor{blue}{bounds} \\
% 30 & 16 & 0.25 & 0.75 & 14 & best & nan & 2 & True & bin & nan & False & 0.433995 & \textcolor{blue}{bounds} \\
% 30 & 17 & 0.50 & 0.50 & 60 & target & pbest & 1 & False & bin & nan & True & 0.497815 & - \\
% 30 & 18 & 0.50 & 0.75 & 60 & target & pbest & 1 & False & bin & nan & True & 0.459689 & \textcolor{red}{centre} \\
% 30 & 19 & 0.25 & 1.00 & 14 & target & best & 1 & False & bin & shade & False & 0.459233 & \textcolor{red}{centre} \\
% 30 & 20 & 0.25 & 0.25 & 14 & best & rand & 2 & False & bin & nan & False & 0.472318 & - \\
% 30 & 21 & 0.25 & 0.50 & 60 & target & best & 1 & True & bin & shade & True & 0.503991 & \textcolor{red}{centre} \\
% 30 & 22 & 1.75 & 0.05 & 14 & target & best & 1 & True & bin & jDE & False & 0.460824 & - \\
% 30 & 23 & 0.25 & 1.00 & 14 & best & nan & 2 & True & exp & shade & False & 0.481032 & \textcolor{blue}{bounds} \\
% 30 & 24 & 0.50 & 0.75 & 14 & best & rand & 1 & False & exp & shade & False & 0.352221 & \textcolor{blue}{bounds} \\
\bottomrule
\end{tabular}}
\end{table} 



==> hallOfFame/de.tex <==
\begin{tabular}{rrrrrllrrllrr}
\toprule
dim & fid & F & CR & lambda_ & mutation_base & mutation_reference & mutation_n_comps & use_archive & crossover & adaptation_method & lpsr & auc \\
\midrule
5 & 1 & 0.250000 & 0.500000 & 8 & best & pbest & 2 & False & bin & shade & False & 0.974087 \\
5 & 1 & 0.250000 & 0.500000 & 10 & best & rand & 2 & False & bin & nan & False & 0.973439 \\
5 & 1 & 0.250000 & 0.500000 & 8 & best & rand & 2 & True & bin & nan & False & 0.973851 \\
5 & 1 & 0.250000 & 0.750000 & 8 & best & rand & 2 & True & exp & nan & False & 0.973927 \\
5 & 1 & 0.250000 & 0.250000 & 8 & best & nan & 2 & True & bin & nan & False & 0.972835 \\
5 & 2 & 0.250000 & 0.250000 & 8 & best & rand & 2 & True & bin & nan & False & 0.944182 \\
5 & 2 & 0.250000 & 0.750000 & 8 & best & pbest & 1 & False & bin & jDE & False & 0.944300 \\
5 & 2 & 0.250000 & 0.050000 & 8 & best & nan & 1 & True & bin & nan & False & 0.947153 \\
5 & 2 & 0.250000 & 0.500000 & 10 & best & pbest & 1 & False & bin & shade & False & 0.947468 \\
5 & 2 & 0.250000 & 0.250000 & 8 & best & rand & 1 & True & bin & nan & False & 0.945785 \\
5 & 3 & 0.750000 & 0.250000 & 8 & target & best & 1 & False & exp & shade & False & 0.909118 \\
5 & 3 & 0.250000 & 0.250000 & 8 & rand & nan & 2 & True & exp & shade & False & 0.905715 \\
5 & 3 & 0.250000 & 0.250000 & 8 & rand & nan & 2 & True & bin & shade & False & 0.908723 \\
5 & 3 & 0.500000 & 0.050000 & 8 & target & pbest & 1 & True & bin & nan & False & 0.908560 \\
5 & 3 & 0.750000 & 0.050000 & 8 & target & best & 1 & False & bin & shade & False & 0.918200 \\
5 & 4 & 0.500000 & 0.250000 & 8 & target & best & 2 & True & exp & nan & False & 0.872835 \\
5 & 4 & 0.250000 & 0.250000 & 8 & rand & nan & 2 & True & exp & shade & False & 0.891569 \\
5 & 4 & 0.750000 & 0.050000 & 8 & target & pbest & 1 & True & exp & shade & False & 0.864715 \\
5 & 4 & 0.500000 & 0.050000 & 10 & best & nan & 2 & True & exp & shade & True & 0.881335 \\
5 & 4 & 0.500000 & 0.050000 & 8 & target & best & 1 & True & exp & nan & False & 0.888952 \\
5 & 5 & 1.750000 & 1.000000 & 8 & best & pbest & 2 & True & bin & shade & False & 0.998437 \\
5 & 5 & 1.750000 & 1.000000 & 8 & best & best & 2 & False & bin & nan & False & 0.998427 \\
5 & 5 & 1.250000 & 0.750000 & 8 & best & pbest & 2 & False & exp & shade & False & 0.998123 \\
5 & 5 & 1.750000 & 0.750000 & 8 & best & best & 1 & True & bin & nan & False & 0.997906 \\
5 & 5 & 1.750000 & 0.750000 & 8 & best & best & 1 & True & bin & nan & False & 0.997748 \\
5 & 6 & 0.500000 & 1.000000 & 8 & target & best & 1 & True & bin & jDE & False & 0.901877 \\
5 & 6 & 0.250000 & 0.750000 & 10 & target & best & 2 & True & bin & shade & True & 0.902323 \\
5 & 6 & 1.250000 & 0.050000 & 8 & target & best & 1 & True & bin & jDE & False & 0.891169 \\
5 & 6 & 0.500000 & 0.500000 & 8 & target & pbest & 2 & True & bin & shade & False & 0.880159 \\
5 & 6 & 0.250000 & 0.750000 & 10 & target & best & 2 & True & bin & shade & True & 0.903013 \\
5 & 7 & 0.250000 & 0.750000 & 10 & target & pbest & 2 & False & bin & shade & True & 0.933372 \\
5 & 7 & 0.750000 & 0.750000 & 10 & target & rand & 1 & False & exp & nan & True & 0.942730 \\
5 & 7 & 0.750000 & 0.500000 & 10 & target & pbest & 1 & False & bin & shade & False & 0.943772 \\
5 & 7 & 0.750000 & 0.750000 & 8 & target & pbest & 1 & True & bin & jDE & False & 0.932748 \\
5 & 7 & 1.750000 & 0.250000 & 10 & target & pbest & 1 & False & bin & jDE & False & 0.936973 \\
5 & 8 & 0.250000 & 0.750000 & 8 & target & pbest & 2 & True & exp & shade & False & 0.895802 \\
5 & 8 & 1.250000 & 0.050000 & 10 & target & best & 1 & False & exp & jDE & False & 0.872810 \\
5 & 8 & 0.500000 & 0.050000 & 8 & best & nan & 1 & True & bin & jDE & False & 0.891419 \\
5 & 8 & 0.250000 & 0.750000 & 10 & best & pbest & 2 & True & bin & shade & True & 0.887259 \\
5 & 8 & 0.250000 & 0.750000 & 10 & best & rand & 1 & True & exp & shade & False & 0.906199 \\
5 & 9 & 0.500000 & 1.000000 & 8 & target & pbest & 1 & True & bin & shade & False & 0.859756 \\
5 & 9 & 0.250000 & 0.750000 & 10 & best & pbest & 2 & True & exp & shade & False & 0.883162 \\
5 & 9 & 0.250000 & 0.750000 & 10 & best & pbest & 2 & True & bin & nan & True & 0.846058 \\
5 & 9 & 0.250000 & 1.000000 & 10 & best & rand & 1 & True & bin & shade & False & 0.870494 \\
5 & 9 & 1.750000 & 0.050000 & 8 & best & nan & 1 & True & bin & jDE & False & 0.878313 \\
5 & 10 & 0.500000 & 1.000000 & 50 & best & pbest & 1 & False & exp & nan & True & 0.804952 \\
5 & 10 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & exp & nan & True & 0.824370 \\
5 & 10 & 0.250000 & 1.000000 & 8 & target & nan & 2 & True & bin & nan & False & 0.835660 \\
5 & 10 & 0.500000 & 1.000000 & 10 & target & best & 2 & True & exp & shade & True & 0.812754 \\
5 & 10 & 0.500000 & 1.000000 & 10 & target & best & 2 & True & exp & shade & False & 0.813252 \\
5 & 11 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & bin & nan & True & 0.874000 \\
5 & 11 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & bin & nan & False & 0.854058 \\
5 & 11 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & bin & nan & False & 0.879245 \\
5 & 11 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & bin & shade & False & 0.872437 \\
5 & 11 & 0.500000 & 1.000000 & 10 & best & rand & 1 & True & bin & nan & True & 0.869298 \\
5 & 12 & 0.250000 & 0.500000 & 10 & target & best & 1 & True & bin & shade & False & 0.536721 \\
5 & 12 & 0.250000 & 0.750000 & 10 & target & pbest & 2 & True & bin & shade & True & 0.768023 \\
5 & 12 & 0.250000 & 0.750000 & 10 & best & nan & 2 & True & bin & shade & True & 0.522095 \\
5 & 12 & 0.500000 & 1.000000 & 10 & target & rand & 2 & True & bin & shade & False & 0.717361 \\
5 & 12 & 0.500000 & 1.000000 & 10 & target & best & 2 & True & bin & shade & True & 0.697311 \\
5 & 13 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & bin & nan & False & 0.768272 \\
5 & 13 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & exp & nan & True & 0.783432 \\
5 & 13 & 0.500000 & 1.000000 & 50 & target & best & 1 & False & bin & nan & False & 0.758036 \\
5 & 13 & 0.500000 & 1.000000 & 8 & best & rand & 1 & True & bin & nan & False & 0.806313 \\
5 & 13 & 0.500000 & 1.000000 & 8 & best & rand & 1 & True & bin & nan & False & 0.816850 \\
5 & 14 & 0.250000 & 0.750000 & 8 & target & pbest & 2 & True & exp & shade & False & 0.921871 \\
5 & 14 & 0.500000 & 1.000000 & 10 & best & pbest & 1 & True & bin & nan & False & 0.912239 \\
5 & 14 & 0.500000 & 1.000000 & 10 & target & pbest & 2 & True & exp & shade & False & 0.909654 \\
5 & 14 & 0.500000 & 1.000000 & 10 & target & best & 2 & True & exp & nan & False & 0.910049 \\
5 & 14 & 0.500000 & 1.000000 & 8 & best & rand & 1 & True & bin & nan & False & 0.915183 \\
5 & 15 & 0.750000 & 1.000000 & 10 & target & pbest & 1 & True & bin & jDE & True & 0.492231 \\
5 & 15 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & bin & shade & True & 0.423966 \\
5 & 15 & 0.250000 & 0.050000 & 10 & best & rand & 1 & False & bin & jDE & False & 0.480284 \\
5 & 15 & 1.750000 & 0.250000 & 8 & target & pbest & 2 & False & bin & jDE & False & 0.562986 \\
5 & 15 & 1.750000 & 0.050000 & 10 & best & rand & 1 & True & bin & jDE & True & 0.511536 \\
5 & 16 & 0.250000 & 1.000000 & 50 & rand & pbest & 1 & False & exp & shade & True & 0.611213 \\
5 & 16 & 0.250000 & 1.000000 & 50 & best & pbest & 2 & True & bin & nan & True & 0.659725 \\
5 & 16 & 0.250000 & 1.000000 & 10 & target & best & 1 & True & exp & shade & False & 0.598848 \\
5 & 16 & 0.500000 & 1.000000 & 10 & target & best & 1 & True & exp & shade & False & 0.618554 \\
5 & 16 & 0.250000 & 1.000000 & 8 & best & rand & 1 & True & bin & nan & True & 0.642246 \\
5 & 17 & 0.250000 & 0.750000 & 10 & rand & rand & 1 & True & exp & nan & False & 0.730496 \\
5 & 17 & 0.500000 & 1.000000 & 8 & rand & rand & 1 & False & bin & jDE & False & 0.736417 \\
5 & 17 & 0.500000 & 0.500000 & 8 & rand & rand & 1 & False & bin & jDE & False & 0.772456 \\
5 & 17 & 0.250000 & 0.050000 & 10 & rand & pbest & 1 & False & bin & jDE & False & 0.727945 \\
5 & 17 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & exp & nan & True & 0.725304 \\
5 & 18 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & bin & nan & True & 0.696950 \\
5 & 18 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & bin & nan & True & 0.680034 \\
5 & 18 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & bin & nan & True & 0.721882 \\
5 & 18 & 0.500000 & 1.000000 & 50 & target & best & 1 & False & exp & nan & False & 0.697552 \\
5 & 18 & 0.500000 & 1.000000 & 50 & target & pbest & 1 & False & bin & nan & False & 0.650480 \\
5 & 19 & 0.250000 & 1.000000 & 8 & best & rand & 2 & False & bin & shade & True & 0.363094 \\
5 & 19 & 0.250000 & 1.000000 & 8 & rand & rand & 2 & True & bin & shade & False & 0.374621 \\
5 & 19 & 0.250000 & 0.750000 & 10 & best & nan & 1 & True & exp & jDE & False & 0.416478 \\
5 & 19 & 0.500000 & 0.750000 & 10 & target & best & 2 & False & bin & shade & False & 0.381884 \\
5 & 19 & 0.250000 & 0.050000 & 8 & best & nan & 1 & True & bin & jDE & False & 0.410125 \\
5 & 20 & 0.250000 & 1.000000 & 10 & best & pbest & 1 & True & exp & jDE & True & 0.854410 \\
5 & 20 & 0.500000 & 1.000000 & 10 & rand & nan & 1 & True & exp & jDE & True & 0.864383 \\
5 & 20 & 0.250000 & 0.050000 & 10 & target & best & 1 & True & exp & jDE & True & 0.825217 \\
5 & 20 & 0.500000 & 0.500000 & 10 & best & pbest & 1 & False & bin & jDE & False & 0.855410 \\
5 & 20 & 1.250000 & 0.250000 & 8 & rand & nan & 2 & True & exp & jDE & False & 0.844259 \\
5 & 21 & 0.250000 & 0.750000 & 8 & rand & best & 1 & True & bin & shade & False & 0.959467 \\
5 & 21 & 1.250000 & 0.250000 & 8 & best & nan & 2 & True & exp & jDE & False & 0.956492 \\
5 & 21 & 0.500000 & 0.750000 & 8 & rand & nan & 1 & True & bin & shade & False & 0.951472 \\
5 & 21 & 0.250000 & 0.750000 & 8 & rand & nan & 2 & True & bin & shade & False & 0.950398 \\
5 & 21 & 1.750000 & 0.750000 & 8 & target & best & 1 & True & bin & jDE & False & 0.950125 \\
5 & 22 & 0.250000 & 1.000000 & 8 & target & pbest & 2 & True & bin & shade & False & 0.933594 \\
5 & 22 & 0.250000 & 0.750000 & 8 & best & pbest & 2 & True & bin & nan & False & 0.928731 \\
5 & 22 & 0.500000 & 1.000000 & 8 & target & pbest & 1 & True & exp & shade & False & 0.941413 \\
5 & 22 & 0.500000 & 0.750000 & 10 & target & best & 1 & True & exp & shade & True & 0.927973 \\
5 & 22 & 1.750000 & 0.250000 & 8 & best & best & 1 & True & bin & jDE & False & 0.889830 \\
5 & 23 & 0.500000 & 1.000000 & 10 & target & best & 1 & True & exp & shade & False & 0.323166 \\
5 & 23 & 0.250000 & 1.000000 & 8 & target & rand & 2 & False & exp & shade & False & 0.279222 \\
5 & 23 & 0.250000 & 1.000000 & 50 & target & pbest & 1 & False & exp & shade & True & 0.379770 \\
5 & 23 & 1.250000 & 1.000000 & 50 & target & best & 1 & False & exp & shade & False & 0.273461 \\
5 & 23 & 0.250000 & 1.000000 & 10 & rand & nan & 2 & True & exp & shade & False & 0.318358 \\
5 & 24 & 0.250000 & 0.750000 & 10 & rand & nan & 1 & True & exp & shade & True & 0.151155 \\
5 & 24 & 0.250000 & 0.750000 & 10 & rand & best & 1 & False & exp & shade & True & 0.175719 \\
5 & 24 & 1.250000 & 0.050000 & 10 & target & best & 1 & False & exp & jDE & False & 0.136960 \\
5 & 24 & 0.500000 & 1.000000 & 50 & target & best & 1 & False & exp & nan & True & 0.139917 \\
5 & 24 & 0.250000 & 0.750000 & 10 & target & rand & 1 & True & bin & shade & True & 0.135802 \\
30 & 1 & 0.250000 & 0.250000 & 14 & rand & pbest & 1 & True & bin & nan & False & 0.672800 \\
30 & 1 & 0.250000 & 0.250000 & 14 & best & rand & 1 & True & bin & shade & False & 0.683745 \\
30 & 1 & 0.250000 & 0.500000 & 14 & rand & pbest & 1 & True & bin & nan & False & 0.684584 \\
30 & 1 & 0.500000 & 0.250000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.669651 \\
30 & 1 & 0.250000 & 0.250000 & 14 & best & rand & 2 & True & bin & shade & False & 0.685956 \\
30 & 2 & 0.750000 & 0.250000 & 14 & target & pbest & 1 & False & bin & nan & False & 0.380647 \\
30 & 2 & 0.750000 & 0.250000 & 14 & target & best & 1 & False & bin & nan & False & 0.378475 \\
30 & 2 & 0.250000 & 0.250000 & 14 & rand & pbest & 2 & True & bin & nan & False & 0.379801 \\
30 & 2 & 0.250000 & 0.250000 & 14 & rand & best & 2 & True & bin & nan & False & 0.367412 \\
30 & 2 & 0.750000 & 0.250000 & 14 & target & pbest & 1 & False & bin & nan & False & 0.366382 \\
30 & 3 & 0.500000 & 0.250000 & 14 & rand & nan & 1 & True & exp & nan & False & 0.101560 \\
30 & 3 & 0.250000 & 0.050000 & 14 & rand & nan & 1 & False & exp & shade & False & 0.107240 \\
30 & 3 & 0.250000 & 0.050000 & 14 & rand & nan & 2 & False & exp & nan & False & 0.096611 \\
30 & 3 & 0.500000 & 0.050000 & 14 & best & nan & 1 & True & exp & shade & False & 0.101129 \\
30 & 3 & 0.250000 & 0.250000 & 14 & rand & nan & 2 & False & exp & nan & False & 0.126384 \\
30 & 4 & 0.500000 & 0.050000 & 14 & rand & nan & 1 & True & exp & shade & False & 0.066849 \\
30 & 4 & 0.250000 & 0.050000 & 14 & rand & nan & 1 & True & exp & shade & False & 0.066764 \\
30 & 4 & 0.250000 & 0.050000 & 14 & rand & nan & 2 & False & exp & nan & False & 0.068164 \\
30 & 4 & 0.500000 & 0.050000 & 14 & rand & nan & 1 & False & exp & shade & False & 0.075975 \\
30 & 4 & 0.500000 & 0.050000 & 14 & rand & nan & 1 & True & exp & shade & False & 0.077353 \\
30 & 5 & 1.750000 & 0.500000 & 14 & best & best & 2 & True & bin & nan & False & 0.972596 \\
30 & 5 & 1.750000 & 0.500000 & 14 & target & pbest & 1 & True & bin & nan & False & 0.974583 \\
30 & 5 & 0.750000 & 0.500000 & 14 & best & best & 2 & False & bin & nan & False & 0.974672 \\
30 & 5 & 1.250000 & 0.750000 & 14 & best & best & 2 & True & bin & shade & False & 0.975968 \\
30 & 5 & 1.750000 & 0.500000 & 14 & best & pbest & 1 & False & bin & nan & False & 0.969127 \\
30 & 6 & 0.250000 & 0.750000 & 14 & target & rand & 2 & True & bin & jDE & False & 0.067959 \\
30 & 6 & 1.250000 & 0.050000 & 14 & target & pbest & 2 & True & bin & jDE & False & 0.055529 \\
30 & 6 & 0.250000 & 0.750000 & 60 & target & pbest & 2 & True & bin & shade & True & 0.050573 \\
30 & 6 & 1.250000 & 1.000000 & 14 & target & rand & 2 & True & bin & jDE & False & 0.053664 \\
30 & 6 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & True & bin & nan & True & 0.059828 \\
30 & 7 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.077297 \\
30 & 7 & 0.500000 & 1.000000 & 14 & target & pbest & 1 & True & bin & shade & True & 0.075933 \\
30 & 7 & 0.750000 & 0.050000 & 14 & target & pbest & 2 & True & bin & jDE & False & 0.081940 \\
30 & 7 & 0.250000 & 0.750000 & 60 & target & pbest & 2 & True & bin & nan & False & 0.085799 \\
30 & 7 & 0.250000 & 0.750000 & 60 & target & pbest & 2 & True & bin & nan & True & 0.087504 \\
30 & 8 & 0.250000 & 0.050000 & 14 & target & best & 1 & True & bin & shade & False & 0.054801 \\
30 & 8 & 0.250000 & 0.050000 & 14 & target & rand & 1 & True & bin & shade & False & 0.056953 \\
30 & 8 & 0.250000 & 0.250000 & 14 & best & nan & 2 & True & bin & shade & False & 0.043725 \\
30 & 8 & 0.250000 & 0.500000 & 14 & target & best & 2 & True & bin & jDE & False & 0.049103 \\
30 & 8 & 0.500000 & 0.750000 & 14 & rand & nan & 1 & True & exp & shade & False & 0.059680 \\
30 & 9 & 0.500000 & 0.500000 & 14 & target & rand & 1 & True & bin & nan & False & 0.043882 \\
30 & 9 & 0.500000 & 1.000000 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.042887 \\
30 & 9 & 0.500000 & 0.750000 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.044560 \\
30 & 9 & 0.500000 & 0.250000 & 14 & target & pbest & 1 & True & bin & nan & False & 0.046263 \\
30 & 9 & 0.500000 & 0.500000 & 14 & target & rand & 1 & True & bin & nan & False & 0.043938 \\
30 & 10 & 0.250000 & 0.050000 & 14 & best & best & 1 & False & bin & jDE & False & 0.000100 \\
30 & 10 & 0.250000 & 0.050000 & 14 & best & best & 1 & False & bin & jDE & False & 0.000100 \\
30 & 10 & 0.250000 & 0.050000 & 14 & best & best & 1 & False & bin & jDE & False & 0.000100 \\
30 & 10 & 0.250000 & 0.050000 & 14 & best & best & 1 & False & bin & jDE & False & 0.000100 \\
30 & 10 & 0.250000 & 0.050000 & 14 & best & best & 1 & False & bin & jDE & False & 0.000100 \\
30 & 11 & 0.250000 & 1.000000 & 300 & target & pbest & 2 & True & exp & nan & True & 0.045241 \\
30 & 11 & 0.250000 & 1.000000 & 14 & target & pbest & 2 & True & exp & nan & True & 0.039152 \\
30 & 11 & 0.250000 & 1.000000 & 14 & target & best & 2 & True & bin & nan & True & 0.045187 \\
30 & 11 & 0.250000 & 1.000000 & 14 & target & pbest & 2 & True & exp & nan & True & 0.054025 \\
30 & 11 & 0.250000 & 1.000000 & 14 & target & best & 2 & True & exp & nan & True & 0.035716 \\
30 & 12 & 0.250000 & 0.500000 & 14 & rand & best & 2 & True & bin & nan & False & 0.116077 \\
30 & 12 & 0.250000 & 0.250000 & 14 & best & rand & 2 & True & bin & shade & False & 0.106247 \\
30 & 12 & 0.500000 & 0.250000 & 14 & target & pbest & 2 & True & bin & shade & False & 0.112709 \\
30 & 12 & 0.750000 & 0.250000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.129169 \\
30 & 12 & 0.500000 & 0.050000 & 14 & target & best & 1 & True & bin & shade & False & 0.118875 \\
30 & 13 & 0.750000 & 0.500000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.122982 \\
30 & 13 & 0.500000 & 0.250000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.105524 \\
30 & 13 & 0.500000 & 1.000000 & 14 & target & best & 2 & True & bin & jDE & False & 0.106653 \\
30 & 13 & 0.500000 & 0.050000 & 14 & target & best & 1 & True & bin & shade & False & 0.095342 \\
30 & 13 & 0.500000 & 0.500000 & 14 & best & rand & 1 & False & bin & nan & False & 0.108358 \\
30 & 14 & 0.250000 & 0.250000 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.354116 \\
30 & 14 & 0.500000 & 0.500000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.362724 \\
30 & 14 & 0.500000 & 0.250000 & 14 & target & best & 1 & True & bin & shade & False & 0.354864 \\
30 & 14 & 0.500000 & 0.250000 & 14 & target & pbest & 1 & True & bin & nan & False & 0.363482 \\
30 & 14 & 0.500000 & 0.250000 & 14 & target & pbest & 1 & True & bin & shade & False & 0.349044 \\
30 & 15 & 0.250000 & 0.750000 & 14 & rand & best & 2 & True & bin & shade & False & 0.004079 \\
30 & 15 & 0.250000 & 0.750000 & 14 & rand & pbest & 2 & True & bin & shade & False & 0.003175 \\
30 & 15 & 1.250000 & 0.050000 & 14 & rand & nan & 1 & False & bin & jDE & False & 0.002752 \\
30 & 15 & 0.250000 & 0.750000 & 14 & rand & nan & 1 & True & bin & shade & False & 0.004773 \\
30 & 15 & 1.750000 & 0.750000 & 14 & best & rand & 2 & False & exp & shade & False & 0.003789 \\
30 & 16 & 0.250000 & 0.500000 & 14 & best & best & 1 & True & bin & nan & False & 0.118570 \\
30 & 16 & 0.250000 & 0.750000 & 14 & best & rand & 2 & True & bin & nan & False & 0.109898 \\
30 & 16 & 0.250000 & 1.000000 & 14 & best & nan & 1 & True & bin & jDE & False & 0.102562 \\
30 & 16 & 0.250000 & 0.750000 & 60 & best & pbest & 1 & False & bin & shade & True & 0.100519 \\
30 & 16 & 0.250000 & 0.750000 & 14 & best & rand & 1 & True & bin & nan & False & 0.103545 \\
30 & 17 & 0.500000 & 0.750000 & 14 & target & pbest & 1 & False & bin & nan & True & 0.196551 \\
30 & 17 & 0.500000 & 0.750000 & 14 & target & pbest & 1 & False & bin & nan & True & 0.199464 \\
30 & 17 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & True & bin & nan & True & 0.201485 \\
30 & 17 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & False & bin & shade & True & 0.201964 \\
30 & 17 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.216308 \\
30 & 18 & 0.500000 & 0.750000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.150361 \\
30 & 18 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.142497 \\
30 & 18 & 0.500000 & 0.500000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.135358 \\
30 & 18 & 0.500000 & 0.750000 & 60 & target & pbest & 1 & False & bin & nan & True & 0.142927 \\
30 & 18 & 0.750000 & 0.750000 & 60 & target & pbest & 1 & False & bin & shade & True & 0.142567 \\
30 & 19 & 0.250000 & 1.000000 & 14 & target & best & 1 & False & bin & shade & False & 0.142203 \\
30 & 19 & 0.250000 & 1.000000 & 14 & target & pbest & 1 & False & bin & shade & False & 0.141115 \\
30 & 19 & 0.250000 & 1.000000 & 14 & target & pbest & 1 & False & exp & shade & False & 0.137516 \\
30 & 19 & 0.250000 & 1.000000 & 14 & target & pbest & 1 & False & bin & shade & False & 0.133953 \\
30 & 19 & 0.250000 & 1.000000 & 14 & target & pbest & 2 & False & bin & shade & False & 0.139599 \\
30 & 20 & 0.250000 & 0.500000 & 14 & rand & nan & 1 & False & exp & shade & False & 0.175146 \\
30 & 20 & 0.500000 & 0.750000 & 14 & best & nan & 1 & True & exp & nan & False & 0.175003 \\
30 & 20 & 0.750000 & 0.750000 & 14 & rand & nan & 1 & False & exp & jDE & False & 0.175688 \\
30 & 20 & 0.250000 & 0.750000 & 14 & rand & nan & 1 & True & exp & nan & False & 0.175908 \\
30 & 20 & 0.500000 & 0.500000 & 14 & best & nan & 1 & False & exp & shade & False & 0.174459 \\
30 & 21 & 1.250000 & 0.750000 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.462257 \\
30 & 21 & 0.250000 & 0.250000 & 60 & best & rand & 1 & False & bin & jDE & True & 0.280085 \\
30 & 21 & 1.250000 & 0.250000 & 14 & target & pbest & 1 & True & bin & jDE & False & 0.353402 \\
30 & 21 & 0.250000 & 0.500000 & 14 & rand & pbest & 1 & True & bin & shade & False & 0.423116 \\
30 & 21 & 0.250000 & 0.500000 & 14 & target & best & 2 & True & bin & shade & False & 0.377283 \\
30 & 22 & 0.250000 & 0.500000 & 60 & best & pbest & 1 & True & bin & nan & True & 0.160409 \\
30 & 22 & 0.500000 & 0.250000 & 14 & target & best & 2 & True & bin & jDE & False & 0.165684 \\
30 & 22 & 0.250000 & 0.250000 & 14 & best & rand & 2 & True & bin & nan & False & 0.197710 \\
30 & 22 & 1.750000 & 0.750000 & 14 & target & rand & 2 & True & bin & jDE & False & 0.158743 \\
30 & 22 & 1.750000 & 0.050000 & 14 & target & best & 1 & True & bin & jDE & False & 0.160424 \\
30 & 23 & 0.250000 & 1.000000 & 14 & best & pbest & 1 & True & exp & shade & False & 0.172326 \\
30 & 23 & 0.250000 & 1.000000 & 14 & best & pbest & 1 & False & bin & shade & False & 0.174680 \\
30 & 23 & 0.250000 & 1.000000 & 14 & best & pbest & 1 & True & exp & shade & False & 0.172572 \\
30 & 23 & 0.250000 & 1.000000 & 14 & best & best & 1 & False & exp & shade & False & 0.176950 \\
30 & 23 & 0.250000 & 1.000000 & 14 & best & nan & 2 & True & exp & shade & False & 0.178161 \\
30 & 24 & 0.750000 & 0.750000 & 14 & target & best & 1 & False & exp & shade & False & 0.000478 \\
30 & 24 & 0.250000 & 0.750000 & 14 & best & rand & 1 & True & exp & shade & False & 0.001390 \\
30 & 24 & 1.250000 & 0.750000 & 14 & best & nan & 1 & True & exp & shade & False & 0.000586 \\
30 & 24 & 0.500000 & 1.000000 & 14 & best & rand & 2 & False & exp & shade & False & 0.000200 \\
30 & 24 & 0.500000 & 0.750000 & 14 & best & nan & 2 & True & exp & shade & False & 0.000700 \\
\bottomrule
\end{tabular}


==> tikz.tex <==
\begin{figure}[!bht]
    \centering
    \begin{tikzpicture}[scale=.4]
        \node (A) at (0, 0) {identify possible uniformity deficiencies, \ref{sect:SB_types}};
        \node (B) at (0, -1.5) {assemble set of data sampling scenarios, \ref{sect:data_gen}};
        \node (C) at (0, -3) {assemble set of statistical sets, \ref{sect:tests}};
        \node (D) at (0, -4.5) {study impact of sample size, \ref{sect:sample_size}};
        \node (E) at (0, -6) {study impact of multiple comparison correction methods, \ref{sect:corrections}};
        \node (F) at (0, -7.5) {study interplay between tests and scenarios, \ref{sect:interplay}};
        \node (G) at (0, -9) {study impact of correlated samples, \ref{sect:correlated}};
        \node (H) at (0, -10.5) {estimate SB type, \ref{sec:rf_model}};
        \node (I) at (0, -12) {finalise \textit{BIAS} toolbox, \ref{sec:toolbox}};
        \node (J) at (0, -13.5) {apply \textit{BIAS} toolbox to algorithmic data, \ref{sect:real-world}};
        \draw[-latex,blue] (A) edge (B); 
        \draw[-latex,blue] (B) edge (C); 
        \draw[-latex,blue] (C) edge (D); 
        \draw[-latex,blue] (D) edge (E); 
        \draw[-latex,blue] (E) edge (F); 
        \draw[-latex,blue] (F) edge (G); 
        \draw[-latex,blue] (G) edge (H); 
        \draw[-latex,blue] (H) edge (I);
        \draw[-latex,blue] (I) edge (J);
    \end{tikzpicture}
    %\vspace{-5mm}
    \caption{Structure of this paper, with Section numbers. \ak{is this figure useful?}\dv{I'm not sure about this, it looks a bit strange to me to have this as a figure instead of just in text}}\label{fig:explain}
\end{figure}

